Towards Holographic Quantum Energy Teleportation

We propose a simplified protocol of quantum energy teleportation (QET) for holographic conformal field theory (CFT) in 3-dimensional anti-de Sitter space with or without black hole. As a tentative proposal, we simplify the standard QET by replacing Alice's local measurement with the local projection, which excites the system from ground state into a particular state dual to a Banados geometry. We then mimic Bob's local operation of the usual QET for extracting energy by deforming the UV surface with a local bump. Adopting the surface/state duality this deformation corresponds to local unitary. We evaluate the extraction of energy from the holographic stress tensor, and find that Bob always gains energy extraction in our protocol. This could be related to the positive energy theorem of the dual gravity. Moreover, the ratio of extraction energy to injection one is a universal function of the UV surface deformation profile.

==> pst-fp.tex <==
%% $Id: pst-fp.tex 837 2013-10-22 07:53:07Z herbert $
%%
%%
%% This is file `pst-fp.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-fp.tex'
%%
%% Herbert Voss <hvoss@tug.org>
%% stolen from the fp package by Michael Mehlich
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-fp' is a PSTricks related package for a division, 
%%    multiplication and addition
%%
\csname PSTFPloaded\endcsname
\let\PSTFPloaded\endinput
%
% Requires some packages
\ifx\PSTricksLoaded\endinput\else\input pstricks \fi
%
\def\fileversion{0.05}
\def\filedate{2010/01/17}
\message{`pst-fp' v\fileversion, \filedate\space (hv)}
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax

%fixed point arithmetic with values between (including)
%      -999999999999999999.999999999999999999
% and  +999999999999999999.999999999999999999

\def\pstFPadd#1#2#3{\pstFP@callc\pstFP@add#1{#2}{#3}+\relax} % #1 := #2+#3
\def\pstFPsub#1#2#3{\pstFP@callc\pstFP@add#1{#2}{-#3}-\relax}% #1 := #2-#3
\def\pstFPmul#1#2#3{\pstFP@callc\pstFP@mul#1{#2}{#3}}        % #1 := #2*#3
\def\pstFPdiv#1#2#3{\pstFP@callc\pstFP@div#1{#2}{#3}}        % #1 := #2/#3

\def\pst@int#1{\expandafter\pst@@int#1..\@nil}
\def\pst@@int#1.#2.\@nil{#1}
\def\pst@Int#1{%
  \@tempdima=#1\relax%
  \expandafter\pst@@Int\the\@tempdima\@nil}
\def\pst@@Int#1.#2\@nil{#1}

%
\def\pstFPMul#1#2#3{\pstFP@callc\pstFP@mul#1{#2}{#3}%        % #1 := int(#2*#3)
  \edef#1{\pst@int{#1}}}%
\def\pstFPDiv#1#2#3{\pstFP@callc\pstFP@div#1{#2}{#3}%        % #1 := int(#2/#3)
  \edef#1{\pst@int{#1}}}%
\def\pstFPstripZeros#1#2{\pst@dimm=#1pt\relax \edef#2{\strip@pt\pst@dimm}}
%
\countdef\pstFP@actcounter=10 % register 0 for counter
\ifnum\pstFP@actcounter<60\relax \pstFP@actcounter=60\fi

\newcount\pstFP@xs %sign of 1st value
\newcount\pstFP@xia%integer part of 1st value
\newcount\pstFP@xib%integer part of 1st value
\newcount\pstFP@xfa%fractional part of 1st value
\newcount\pstFP@xfb%fractional part of 1st value

\countdef\pstFP@ys=5 %sign of 2nd value
\countdef\pstFP@yia=6%integer part of 2nd value
\countdef\pstFP@yib=7%integer part of 2nd value
\countdef\pstFP@yfa=8%fractional part of 2nd value
\countdef\pstFP@yfb=9%fractional part of 2nd value

\countdef\pstFP@xk=10  %registers for splitting 1st value
\countdef\pstFP@xl=11
\countdef\pstFP@xm=12
\countdef\pstFP@xn=13
\countdef\pstFP@xo=14
\countdef\pstFP@xp=15
\countdef\pstFP@xq=16
\countdef\pstFP@xr=17
\countdef\pstFP@xz=18
\countdef\pstFP@xt=19
\countdef\pstFP@xu=20
\countdef\pstFP@xv=21

\countdef\pstFP@yk=22 %registers for splitting 2nd value
\countdef\pstFP@yl=23
\countdef\pstFP@ym=24
\countdef\pstFP@yn=25
\countdef\pstFP@yo=26
\countdef\pstFP@yp=27
\countdef\pstFP@yq=28
\countdef\pstFP@yr=29
\countdef\pstFP@yz=30
\countdef\pstFP@yt=31
\countdef\pstFP@yu=32
\countdef\pstFP@yv=33

\newcount\pstFP@rega   %auxiliary registers
\newcount\pstFP@regb
\countdef\pstFP@regc=36
\countdef\pstFP@regd=37
\countdef\pstFP@rege=38

\countdef\pstFP@rs=39 %result registers
\countdef\pstFP@ria=40
\countdef\pstFP@rib=41
\countdef\pstFP@rfa=42
\countdef\pstFP@rfb=43

\newcount\pstFP@regs    %local auxiliary registers
\countdef\pstFP@count=45
\countdef\pstFP@res=46
\countdef\pstFP@shift=47
\newcount\pstFP@times
\countdef\pstFP@prod=49

%auxiliary macros which may be used in all of the following macros
\newif\ifpstFP@test

\def\pstFP@ignorenext#1{}
\def\pstFP@first#1#2\relax{#1}
\def\pstFP@swallow#1\relax{}
%
\def\ifpstFP@zero#1{%
  \ifnum%
    \expandafter\ifnum\csname pstFP@#1ia\endcsname=0 0\else1\fi%
    \expandafter\ifnum\csname pstFP@#1ib\endcsname=0 0\else1\fi%
    \expandafter\ifnum\csname pstFP@#1fa\endcsname=0 0\else1\fi%
    \expandafter\ifnum\csname pstFP@#1fb\endcsname=0 0\else1\fi%
    =0\relax%
}
%
%read value
%
\def\pstFP@correctintcounter#1\relax{%
  {\edef\pstFP@tmp{#1}%
   \pstFP@count=0\relax%
   \loop%
     \edef\pstFP@tmpa{\expandafter\pstFP@first\pstFP@tmp\noexpand\relax}%
     \expandafter\ifx\pstFP@tmpa0\relax%
        \advance\pstFP@count1\relax%
        \edef\pstFP@tmp{\expandafter\pstFP@ignorenext\pstFP@tmp}%
     \repeat%
   \ifnum\pstFP@count>18\relax \typeout{>>>> Overflow}\fi%
   \expandafter\if!\pstFP@tmp!%
     \advance\pstFP@count-18\relax%
     \pstFP@count=-\pstFP@count%
     \loop%
       \ifnum\pstFP@count>0\relax%
          \pstFP@regc=\pstFP@rega%
	  \divide\pstFP@rega10\relax\multiply\pstFP@rega10\relax%
	  \advance\pstFP@regc-\pstFP@rega\multiply\pstFP@regc100000000\relax%
	  \divide\pstFP@rega10\relax%
	  \divide\pstFP@regb10\relax\advance\pstFP@regb\pstFP@regc%
	  \advance\pstFP@count-1\relax%
       \repeat%
     \global\pstFP@rega=\pstFP@rega%
     \global\pstFP@regb=\pstFP@regb%
   \else%
     \typeout{>>>>Number too big}%
   \fi%
  }%
}
\def\pstFP@@setintcounter#1#2#3#4#5#6#7#8#9{%
  \pstFP@regb=#1#2#3#4#5#6#7#8#9\relax%
  \pstFP@correctintcounter%
}
\def\pstFP@setintcounter#1#2#3#4#5#6#7#8#9{%
  \pstFP@rega=#1#2#3#4#5#6#7#8#9\relax%
  \pstFP@@setintcounter%
}

\def\pstFP@@setfractcounter#1#2#3#4#5#6#7#8#9{%
  \pstFP@regb=#1#2#3#4#5#6#7#8#9\relax%
  \pstFP@swallow%
}
\def\pstFP@setfractcounter#1#2#3#4#5#6#7#8#9{%
  \pstFP@rega=#1#2#3#4#5#6#7#8#9\relax%
  \pstFP@@setfractcounter%
}

\def\pstFP@getsign#1\relax{%
  {\pstFP@regs=1\relax%
   \edef\pstFP@tmp{#1}%
   \loop%
     \edef\pstFP@tmpa{\expandafter\pstFP@first\pstFP@tmp\noexpand\relax}%
     \expandafter\ifx\pstFP@tmpa-\relax%
        \multiply\pstFP@regs-1\relax%
     \fi%
     \ifnum\expandafter\ifx\pstFP@tmpa-1\else0\fi\expandafter\ifx\pstFP@tmpa+1\else0\fi>0%
        \edef\pstFP@tmp{\expandafter\pstFP@ignorenext\pstFP@tmp}%
     \repeat%
   \global\let\pstFP@tmp\pstFP@tmp%
   \global\pstFP@regs=\pstFP@regs%
  }%
}

\def\pstFP@removeleadingzeros#1\relax{%
  {\edef\pstFP@tmp{#1}%
   \loop%
     \edef\pstFP@tmpa{\expandafter\pstFP@first\pstFP@tmp\noexpand\relax}%
     \expandafter\ifx\pstFP@tmpa0\relax%
       \edef\pstFP@tmp{\expandafter\pstFP@ignorenext\pstFP@tmp}%
     \repeat%
   \global\let\pstFP@tmp\pstFP@tmp%
  }%
}

\newif\ifpstFP@nonstop
\def\pstFP@strip#1{%
  {\edef\pstFP@tmp{#1}%
   \edef\pstFP@tmpb{}%
   \ifx\pstFP@tmp\@empty\else%
     \pstFP@nonstoptrue%
     \loop%
       \edef\pstFP@tmpa{\expandafter\pstFP@first\pstFP@tmp\noexpand\relax}%
       \expandafter\ifx\pstFP@tmpa-\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa+\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa0\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa1\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa2\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa3\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa4\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa5\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa6\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa7\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa8\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa9\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \ifx\pstFP@tmpa\@empty\pstFP@nonstopfalse\else%
       \ifx\pstFP@tmpa\space\pstFP@nonstopfalse\else%
         \typeout{>>> Illegal character \pstFP@tmpa\space found in float number}%
       \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi%
       \edef\pstFP@tmp{\expandafter\pstFP@ignorenext\pstFP@tmp}%
       \ifx\pstFP@tmp\@empty\pstFP@nonstopfalse\fi%
       \ifpstFP@nonstop%
       \repeat%
   \fi%
   \global\let\pstFP@tmp\pstFP@tmpb%
  }%
}

\def\pstFP@readvalue#1#2#3{%
  % #1    macro family to catch the value
  % #2.#3 value
  %
  % regular expression [+|-]*[d]_0^18.[d]*
  %
  \pstFP@strip{#2}%
  %sign
  \expandafter\pstFP@getsign\pstFP@tmp\relax%
  \csname pstFP@#1s\endcsname=\pstFP@regs%
  %
  %integer part
  \pstFP@removeleadingzeros\pstFP@tmp\relax%
  \expandafter\pstFP@setintcounter\pstFP@tmp000000000000000000\relax%
  \csname pstFP@#1ia\endcsname=\pstFP@rega%
  \csname pstFP@#1ib\endcsname=\pstFP@regb%
  %
  %fractional part
  \pstFP@strip{#3}%
  \expandafter\pstFP@setfractcounter\pstFP@tmp000000000000000000\relax%
  \csname pstFP@#1fa\endcsname=\pstFP@rega%
  \csname pstFP@#1fb\endcsname=\pstFP@regb%
  %
  %correct sign
  \ifnum\pstFP@rega=0\relax%
    \ifnum\pstFP@regb=0\relax%
      \expandafter\ifnum\csname pstFP@#1ib\endcsname=0\relax%
        \expandafter\ifnum\csname pstFP@#1ia\endcsname=0\relax%
	  \csname pstFP@#1s\endcsname=1\relax%
	\fi%
      \fi%
    \fi%
  \fi%
}
%
%store value in macro
%
\def\pstFP@store#1#2{%
  % #1 macro
  % #2 macro family (value) to store
  %
  \ifpstFP@zero{#2}%
    \csname pstFP@#2s\endcsname=1\relax%
  \fi%
  \expandafter\ifnum\csname pstFP@#2s\endcsname<0\relax%
    \edef#1{-}%
  \else%
    \edef#1{}%
  \fi%
  \expandafter\ifnum\csname pstFP@#2ia\endcsname=0\relax%
     \expandafter\ifnum\csname pstFP@#2ib\endcsname=0\relax%
       \edef#1{#10}%
     \else%
       \edef#1{#1\expandafter\the\csname pstFP@#2ib\endcsname}%
     \fi%
  \else%
    \expandafter\advance\csname pstFP@#2ib\endcsname1000000000\relax%
    \edef#1{#1\expandafter\the\csname pstFP@#2ia\endcsname\expandafter\pstFP@ignorenext\the\csname pstFP@#2ib\endcsname}%
  \fi%
  \expandafter\advance\csname pstFP@#2fa\endcsname1000000000\relax%
  \expandafter\advance\csname pstFP@#2fb\endcsname1000000000\relax%
  \edef#1{#1\noexpand.\expandafter\pstFP@ignorenext\the\csname pstFP@#2fa\endcsname\expandafter\pstFP@ignorenext\the\csname pstFP@#2fb\endcsname}%
}
%macros to expand some arguments
%
\def\pstFP@callc#1#2#3#4{%
  % #1 macro to call
  % #2 macro, which gets the result
  % #3 1st value
  % #4 2nd value
  % expand the values and split them into the integer and the fractional parts
  \edef\next{\noexpand#1\noexpand#2#3..\noexpand\relax#4..\noexpand\relax}%
  \next%
}
%
\def\pstFP@divten#1{%
  \expandafter\pstFP@regc\csname pstFP@#1ia\endcsname%
  \expandafter\divide\csname pstFP@#1ia\endcsname10\relax%
  \expandafter\pstFP@regb\csname pstFP@#1ia\endcsname%
  \multiply\pstFP@regb10\relax%
  \advance\pstFP@regc-\pstFP@regb%
  \multiply\pstFP@regc100000000\relax%
  %
  \expandafter\pstFP@rega\csname pstFP@#1ib\endcsname%
  \expandafter\divide\csname pstFP@#1ib\endcsname10\relax%
  \expandafter\pstFP@regb\csname pstFP@#1ib\endcsname%
  \multiply\pstFP@regb10\relax%
  \advance\pstFP@rega-\pstFP@regb%
  \multiply\pstFP@rega100000000\relax%
  \expandafter\advance\csname pstFP@#1ib\endcsname\pstFP@regc%
  %
  \expandafter\pstFP@regc\csname pstFP@#1fa\endcsname%
  \expandafter\divide\csname pstFP@#1fa\endcsname10\relax%
  \expandafter\pstFP@regb\csname pstFP@#1fa\endcsname%
  \multiply\pstFP@regb10\relax%
  \advance\pstFP@regc-\pstFP@regb%
  \multiply\pstFP@regc100000000\relax%
  \expandafter\advance\csname pstFP@#1fa\endcsname\pstFP@rega%
  %
  \expandafter\divide\csname pstFP@#1fb\endcsname10\relax%
  \expandafter\advance\csname pstFP@#1fb\endcsname\pstFP@regc%
}
%
\def\pstFP@multen#1{%
  \expandafter\multiply\csname pstFP@#1ia\endcsname10\relax%
  \expandafter\ifnum\csname pstFP@#1ib\endcsname<100000000\relax%
  \else%
    \expandafter\pstFP@regc\csname pstFP@#1ib\endcsname%
    \divide\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1ia\endcsname\pstFP@regc%
    \multiply\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1ib\endcsname-\pstFP@regc%
  \fi%
  \expandafter\multiply\csname pstFP@#1ib\endcsname10\relax%
  \expandafter\ifnum\csname pstFP@#1fa\endcsname<100000000\relax%
  \else%
    \expandafter\pstFP@regc\csname pstFP@#1fa\endcsname%
    \divide\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1ib\endcsname\pstFP@regc%
    \multiply\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1fa\endcsname-\pstFP@regc%
  \fi%
  \expandafter\multiply\csname pstFP@#1fa\endcsname10\relax%
  \expandafter\ifnum\csname pstFP@#1fb\endcsname<100000000\relax%
  \else%
    \expandafter\pstFP@regc\csname pstFP@#1fb\endcsname%
    \divide\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1fa\endcsname\pstFP@regc%
    \multiply\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1fb\endcsname-\pstFP@regc%
  \fi%
  \expandafter\multiply\csname pstFP@#1fb\endcsname10\relax%
}
%
\def\pstFP@counttimes{%
  {\global\pstFP@times=0\relax%
   \loop%
     \ifnum%
        \ifnum\pstFP@xia>\pstFP@yia1%
	\else\ifnum\pstFP@xia<\pstFP@yia0%
	\else%
	  \ifnum\pstFP@xib>\pstFP@yib1%
	  \else\ifnum\pstFP@xib<\pstFP@yib0%
	  \else%
	    \ifnum\pstFP@xfa>\pstFP@yfa1%
	    \else\ifnum\pstFP@xfa<\pstFP@yfa0%
	    \else%
	      \ifnum\pstFP@xfb>\pstFP@yfb1%
	      \else\ifnum\pstFP@xfb<\pstFP@yfb0%
	      \else%
	         1%
	      \fi\fi%
	    \fi\fi%
	  \fi\fi%
	\fi\fi%
	=1\relax%
       \global\advance\pstFP@times1\relax%
       \global\advance\pstFP@xfb-\pstFP@yfb%
       \ifnum\pstFP@xfb<0\relax%
         \global\advance\pstFP@xfb1000000000\relax%
	 \global\advance\pstFP@xfa-1\relax%
       \fi%
       \global\advance\pstFP@xfa-\pstFP@yfa%
       \ifnum\pstFP@xfa<0\relax%
         \global\advance\pstFP@xfa1000000000\relax%
	 \global\advance\pstFP@xib-1\relax%
       \fi%
       \global\advance\pstFP@xib-\pstFP@yib%
       \ifnum\pstFP@xib<0\relax%
         \global\advance\pstFP@xib1000000000\relax%
	 \global\advance\pstFP@xia-1\relax%
       \fi%
       \global\advance\pstFP@xia-\pstFP@yia%
     \repeat%
  }%
}
%
\def\pstFP@add#1#2.#3.#4\relax#5.#6.#7\relax#8\relax{%
  % #1 macro, which gets the result
  % #2 integer part of 1st value 
  % #3 fractional part of 1st value
  % #4 dummy to swallow everthing after the 2nd '.'
  % #5 integer part of 2nd value 
  % #6 fractional part of 2nd value
  % #7 dummy to swallow everthing after the 2nd '.'
  %
  {\pstFP@readvalue{x}{#2}{#3}%
   \pstFP@readvalue{y}{#5}{#6}%
   %
   \ifnum\pstFP@xs=\pstFP@ys%
     \advance\pstFP@xfb\pstFP@yfb%
     \advance\pstFP@xfa\pstFP@yfa%
     \ifnum\pstFP@xfb<1000000000\relax\else%
       \advance\pstFP@xfb-1000000000\relax%
       \advance\pstFP@xfa1\relax%
     \fi%
     \advance\pstFP@xib\pstFP@yib%
     \ifnum\pstFP@xfa<1000000000\relax\else%
       \advance\pstFP@xfa-1000000000\relax%
       \advance\pstFP@xib1\relax%
     \fi%
     \advance\pstFP@xia\pstFP@yia%
     \ifnum\pstFP@xib<1000000000\relax\else%
       \advance\pstFP@xib-1000000000\relax%
       \advance\pstFP@xia1\relax%
     \fi%
     \ifnum\pstFP@xia<1000000000\relax\else%
       \pstFP@errmessage{Overflow}%
     \fi%
     \pstFP@store\pstFP@tmp{x}%
   \else%
     \advance\pstFP@xfb-\pstFP@yfb%
     \ifnum\pstFP@xfb<0\relax%
       \advance\pstFP@yfa1\relax%
       \advance\pstFP@xfb1000000000\relax%
     \fi%
     \advance\pstFP@xfa-\pstFP@yfa%
     \ifnum\pstFP@xfa<0\relax%
       \advance\pstFP@yib1\relax%
       \advance\pstFP@xfa1000000000\relax%
     \fi%
     \advance\pstFP@xib-\pstFP@yib%
     \ifnum\pstFP@xib<0\relax%
       \advance\pstFP@yia1\relax%
       \advance\pstFP@xib1000000000\relax%
     \fi%
     \advance\pstFP@xia-\pstFP@yia%
     \ifnum\pstFP@xia<0\relax%
       \pstFP@xs=-\pstFP@xs%
       \ifnum\pstFP@xfb=0\relax\else%
         \advance\pstFP@xfb-1000000000\relax\pstFP@xfb=-\pstFP@xfb%
	 \advance\pstFP@xfa1\relax%
       \fi%
       \ifnum\pstFP@xfa=0\relax\else%
         \advance\pstFP@xfa-1000000000\relax\pstFP@xfa=-\pstFP@xfa%
	 \advance\pstFP@xib1\relax%
       \fi%
       \ifnum\pstFP@xib=0\relax\else%
         \advance\pstFP@xib-1000000000\relax\pstFP@xib=-\pstFP@xib%
	 \advance\pstFP@xia1\relax%
       \fi%
       \relax\pstFP@xia=-\pstFP@xia%
     \fi%
     \pstFP@store\pstFP@tmp{x}%
   \fi%
   \global\let\pstFP@tmp\pstFP@tmp%
  }%
  \let#1\pstFP@tmp%
}


\def\pstFP@div#1#2.#3.#4\relax#5.#6.#7\relax{%
  % #1 macro, which gets the result
  % #2 integer part of 1st value 
  % #3 fractional part of 1st value
  % #4 dummy to swallow everthing after the 2nd '.'
  % #5 integer part of 2nd value 
  % #6 fractional part of 2nd value
  % #7 dummy to swallow everthing after the 2nd '.'
  %
  % algorithmic idea (for x>0, y>0)
  %   - %determine \pstFP@shift  such that y*10^\pstFP@shift <100000000<=y*10^(\pstFP@shift+1)
  %   - %determine \pstFP@shift' such that x*10^\pstFP@shift'<100000000<=x*10^(\pstFP@shift+1)
  %   - x=x*\pstFP@shift'
  %   - y=y*\pstFP@shift
  %   - \pstFP@shift=\pstFP@shift-\pstFP@shift'
  %   - res=0
  %   - while y>0 %fixed-point representation!
  %   -   \pstFP@times=0
  %   -	  while x>y
  %   -     \pstFP@times=\pstFP@times+1
  %   -     x=x-y
  %   -   end
  %   -   y=y/10
  %   -   res=10*res+\pstFP@times/1000000000
  %   - end
  %   - %shift the result according to \pstFP@shift
  %
  {\pstFP@readvalue{x}{#2}{#3}%
   \pstFP@readvalue{y}{#5}{#6}%
   %
   %sign
   \multiply\pstFP@xs\pstFP@ys%
   \pstFP@rs=\pstFP@xs%
   %
   %compute division
   \ifpstFP@zero{y}%
     \typeout{>>>>Division by zero}%
   \else%
     \ifpstFP@zero{x}\def\next##1{\edef\pstFP@tmp{0}}\else\def\next##1{##1}\fi%
     \next%
       {\pstFP@shift=0\relax%
        \loop%
          \ifnum\pstFP@yia<100000000\relax%
	     \pstFP@multen{y}%
	     \advance\pstFP@shift1\relax%
	   \repeat%
        \loop%
          \ifnum\pstFP@xia<100000000\relax%
	     \pstFP@multen{x}%
	     \advance\pstFP@shift-1\relax%
	  \repeat%
        \pstFP@ria=0\pstFP@rib=0\pstFP@rfa=0\pstFP@rfb=0\relax%
        \loop%
          \ifpstFP@zero{y}\else%
	     \pstFP@counttimes%divides x by \pstFP@times*y
	     \pstFP@divten{y}%
	     \pstFP@multen{r}%
	     \advance\pstFP@rfb\pstFP@times%
	     \ifnum\pstFP@rfb<1000000000\relax\else%
	       \advance\pstFP@rfa1\advance\pstFP@rfb-1000000000\relax%
	       \ifnum\pstFP@rfa<1000000000\relax\else%
	         \advance\pstFP@rib1\advance\pstFP@rfa-1000000000\relax%
		 \ifnum\pstFP@rib<1000000000\relax\else%
		   \advance\pstFP@ria1\advance\pstFP@rib-1000000000\relax%
		 \fi%
	       \fi%
	     \fi%
	  \repeat%
        \loop%
          \ifnum\pstFP@shift>17%
	    \advance\pstFP@shift-1\relax%
	    \ifnum\pstFP@ria<100000000\else\pstFP@ria=-1\fi%
	    \ifnum\pstFP@ria<0\pstFP@ria=-1\fi%
	    \pstFP@multen{r}%
	  \repeat%
        \ifnum\pstFP@ria<1000000000\else\pstFP@ria=-1\fi%
        \loop%
          \ifnum\pstFP@shift<17%
	    \advance\pstFP@shift1\relax%
	    \pstFP@divten{r}%
	  \repeat%
        \ifnum\pstFP@ria<0\relax%
          \typeout{>>>>Overflow}%
        \else%
          \pstFP@store\pstFP@tmp{r}%
        \fi%
       }%
    \fi%
   %
   \global\let\pstFP@tmp=\pstFP@tmp%
   %
  }%
  \let#1\pstFP@tmp%
}
%multiply two values

\def\pstFP@firstnine#1#2#3#4#5#6#7#8#9{%
  \pstFP@res=#1#2#3#4#5#6#7#8#9\relax%
}
\def\pstFP@@ninesplit#1\relax#2\end#3{%
  #1%
  \edef#3{#2}%
}
\def\pstFP@ninesplit#1{%
  \edef#1{\expandafter\pstFP@firstnine\pstFP@rd}%
  \expandafter\pstFP@@ninesplit#1\end#1\relax%
}

\def\pstFP@split#1#2#3#4{%
  % #1 highest three digits
  % #2 medium three digits
  % #3 least three digits
  % #4 counter
  \pstFP@regc=#4%
  \divide\pstFP@regc1000000\relax%
  #1=\pstFP@regc%
  \multiply\pstFP@regc-1000000\relax\advance\pstFP@regc#4%
  #3=\pstFP@regc%
  \divide\pstFP@regc1000\relax%
  #2=\pstFP@regc%
  \multiply\pstFP@regc-1000\relax\advance\pstFP@regc#3%
  #3=\pstFP@regc%
}

\def\pstFP@@mul#1#2#3{%
  \pstFP@regc=\csname pstFP@x#1\endcsname%
  \multiply\pstFP@regc\csname pstFP@y#2\endcsname%
  \advance\pstFP@prod\pstFP@regc%
  %
  \ifx#3\relax%
    \let\next=\relax% 
  \else%
    \let\next=\pstFP@@mul%
  \fi%
  \next#3%
}

\def\pstFP@saveshift{%
  % save rightmost three digits 
  \pstFP@regc=\pstFP@prod%
  \divide\pstFP@prod1000\relax%
  \multiply\pstFP@prod1000\relax%
  \advance\pstFP@regc-\pstFP@prod%
  \advance\pstFP@regc1000\relax%
  \edef\pstFP@rd{\expandafter\pstFP@ignorenext\the\pstFP@regc\pstFP@rd}%
  %
  \divide\pstFP@prod1000\relax%
}

\def\pstFP@mul#1#2.#3.#4\relax#5.#6.#7\relax{%
  % #1 macro, which gets the result
  % #2 integer part of 1st value 
  % #3 fractional part of 1st value
  % #4 dummy to swallow everthing after the 2nd '.'
  % #5 integer part of 2nd value 
  % #6 fractional part of 2nd value
  % #7 dummy to swallow everthing after the 2nd '.'
  %
  % split value in various parts
  % x y = 123 456 789 123 456 789 . 123 456 789 123 456 789
  % ->    xk  xl  xm  xn  xo  xp    xq  xr  xs  xt  xu  xv
  % ->    yk  yl  ym  yn  yo  yp    yq  yr  ys  yt  yu  yv
  % multiply these parts and save the result wrt the necessary shifts
  %
  {\pstFP@readvalue{x}{#2}{#3}%
   \pstFP@readvalue{y}{#5}{#6}%
   %
   %sign
   \multiply\pstFP@xs\pstFP@ys%
   \pstFP@rs=\pstFP@xs%
   %
   % split parts
   \pstFP@split\pstFP@xk\pstFP@xl\pstFP@xm\pstFP@xia\pstFP@split\pstFP@xn\pstFP@xo\pstFP@xp\pstFP@xib%
   \pstFP@split\pstFP@xq\pstFP@xr\pstFP@xz\pstFP@xfa\pstFP@split\pstFP@xt\pstFP@xu\pstFP@xv\pstFP@xfb%
   \pstFP@split\pstFP@yk\pstFP@yl\pstFP@ym\pstFP@yia\pstFP@split\pstFP@yn\pstFP@yo\pstFP@yp\pstFP@yib%
   \pstFP@split\pstFP@yq\pstFP@yr\pstFP@yz\pstFP@yfa\pstFP@split\pstFP@yt\pstFP@yu\pstFP@yv\pstFP@yfb%
   %
   \pstFP@prod=0\relax%
   \edef\pstFP@rd{}%
   %
   %compute result
   \pstFP@@mul vv 				   \relax\pstFP@saveshift%
   \pstFP@@mul vu uv			           \relax\pstFP@saveshift%
   \pstFP@@mul uu vt tv 			   \relax\pstFP@saveshift%
   \pstFP@@mul ut tu vz zv 		           \relax\pstFP@saveshift%
   \pstFP@@mul tt zu uz rv vr		           \relax\pstFP@saveshift%
   \pstFP@@mul zt tz ur ru vq qv 		   \relax\pstFP@saveshift%
   \pstFP@@mul zz rt tr uq qu vp pv  	           \relax\pstFP@saveshift%
   \pstFP@@mul zr rz tq qt up pu vo ov 	           \relax\pstFP@saveshift%
   \pstFP@@mul rr qz zq tp pt uo ou vn nv 	   \relax\pstFP@saveshift%
   \pstFP@@mul rq qr zp pz to ot un nu vm mv       \relax\pstFP@saveshift%
   \pstFP@@mul qq rp pr zo oz tn nt um mu vl lv    \relax\pstFP@saveshift%
   \pstFP@@mul qp pq ro or zn nz tm mt ul lu kv vk \relax\pstFP@saveshift%
   \pstFP@@mul pp oq qo rn nr zm mz tl lt ku uk    \relax\pstFP@saveshift%
   \pstFP@@mul op po nq qn rm mr zl lz tk kt       \relax\pstFP@saveshift%
   \pstFP@@mul oo pn np mq qm rl lr kz zk          \relax\pstFP@saveshift%
   \pstFP@@mul no on mp pm lq ql kr rk 	           \relax\pstFP@saveshift%
   \pstFP@@mul nn mo om pl lp qk kq 	           \relax\pstFP@saveshift%
   \pstFP@@mul mn nm lo ok pk kp 		   \relax\pstFP@saveshift%
   \pstFP@@mul mm ln nl ko ok 		           \relax\pstFP@saveshift%
   \pstFP@@mul lm ml kn nk			   \relax\pstFP@saveshift%
   \pstFP@@mul ll km mk 			   \relax\pstFP@saveshift%
   \pstFP@@mul kl lk 			           \relax\pstFP@saveshift%
   \pstFP@@mul kk 				   \relax\pstFP@saveshift\pstFP@saveshift%
   \pstFP@ninesplit\pstFP@rd%
   \ifnum\pstFP@res=0\relax%
     \pstFP@ninesplit\pstFP@rd%
     \ifnum\pstFP@res=0\relax%
       \pstFP@ninesplit\pstFP@rd\pstFP@ria=\pstFP@res%
       \pstFP@ninesplit\pstFP@rd\pstFP@rib=\pstFP@res%
       \pstFP@ninesplit\pstFP@rd\pstFP@rfa=\pstFP@res%
       \pstFP@ninesplit\pstFP@rd\pstFP@rfb=\pstFP@res%
       \pstFP@store\pstFP@tmp{r}%
     \else\typeout{pstFPmul: Overflow}\fi%
   \else\typeout{pstFPmul: Overflow}\fi%
   \global\let\pstFP@tmp\pstFP@tmp}%
  \let#1\pstFP@tmp%
}
%
\catcode`\@=\PstAtCode\relax
%
%% END: pst-fp.tex
\endinput


==> pst-node.tex <==
% $Id: pst-node.tex 68 2014-08-07 10:16:26Z herbert $
%%
%% BEGIN pst-node.tex
%%
%% Nodes with PSTricks.
%% This uses the header file `pst-node.pro'.
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%% COPYRIGHT 2009-2015 by Herbert Voss, hvoss tug.org.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
%
\csname PSTnodesLoaded\endcsname
\let\PSTnodesLoaded\endinput
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex \fi\relax
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey \fi
%
\def\fileversion{1.36}
\def\filedate{2016/04/24}
\message{ v\fileversion, \filedate}
%
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
%
\pstheader{pst-node.pro}
\pst@addfams{pst-node}
%
\SpecialCoor
%
%%%%%%%%%% compatibility stuff
\define@boolkey[psset]{pst-node}[Pst@]{trueAngle}[true]{}
\psset[pst-node]{trueAngle=false}
%%%%%%%%%% compatibility stuff
\define@boolkey[psset]{pst-node}[Pst@]{storeNodeInfo}[true]{}
\psset[pst-node]{storeNodeInfo=false}
%
\def\pst@nodedict{tx@NodeDict begin }
\def\pst@zapspace#1 #2{%
#1%
\ifx#2\@empty\else\expandafter\pst@zapspace\fi
#2}
%
\def\pst@getnode#1#2{\pst@expandafter\pst@@getnode{#1},,\@nil#2}
\def\pst@@getnode#1,#2,#3\@nil#4{%
  \ifx\@empty#3\@empty
    \edef#4{/N@\pst@zapspace#1 \@empty\space}%
  \else
    \pst@cntg=#1\relax
    \pst@cnth=#2\relax
    \edef#4{/N@M-\ifnum\psmatrixcnt=\z@ 1\else\the\psmatrixcnt\fi
    -\the\pst@cntg-\the\pst@cnth\space}%
  \fi}
%
% bug fix for xelatex, dvipdfmx uses the wrong scaling
\def\tx@NewNode{/NodeScale {\ifx\pstnodescale\@undefined  \else\pstnodescale \fi} def NewNode }
%
\def\psopenNodeFile{%
  \pst@Verb{ %globaldict begin
%  tx@NodeDict begin 
    (\jobname.nodes) (w) file /NodeFile exch def 
%    end 
  }}
 %
\def\pscloseNodeFile{\pstVerb{ tx@NodeDict begin NodeFile closefile end }}
%
\define@boolkey[psset]{pst-node}[Pst@]{showNode}[true]{\ifPst@showNode\psopenNodeFile\fi}% write coors into the logfile
\define@boolkey[psset]{pst-node}[Pst@]{markNode}[true]{}% makr the node with its name
\define@boolkey[psset]{pst-node}[Pst@]{saveNodeCoors}[true]{}
\define@key[psset]{pst-node}{NodeCoorPrefix}[]{\def\psk@NodeCoorPrefix{#1}}% if empty it is N-<Name>.x|y
\psset[pst-node]{saveNodeCoors=false,showNode=false,markNode=false,NodeCoorPrefix=}% <NodeCoorPrefix<Name>x|y>
%
\def\pst@newnode#1#2#3#4{%
\pst@killglue
\leavevmode
\pst@getnode{#1}\pst@thenode
\pst@Verb{
  \ifPst@saveNodeCoors
    \ifx\relax#3\relax 0 0 \else gsave \pst@dict STV CP T end #3 \tx@UserCoor grestore \fi 
    \if$\psk@NodeCoorPrefix$
      /N-#1.y exch def
      /N-#1.x exch def
    \else
      /\psk@NodeCoorPrefix#1y exch def
      /\psk@NodeCoorPrefix#1x exch def
    \fi
  \fi
  \pst@nodedict
  {#3}
  \ifx\psk@name\relax false \else \psk@name true \fi
  \pst@thenode
  #2
  {#4}
  \ifPst@showNode 
  exch dup /NodeType ED 
  exch
   NodeType 10 eq {  % pnode type
    5 copy 
    cvlit aload pop
    20 string cvs (; )   6 2 roll % InitPnode
    20 string cvs (; )   7 2 roll % type
    20 string cvs (; )   8 2 roll %/N@Name
    20 string cvs (; )   9 2 roll % true/false
    cvlit dup length 2 eq 
      { aload pop exch 
        20 string cvs (; ) 11 2 roll 
        20 string cvs (, ) 12 2 roll  % x,y
        (\string\n)                   % add newline
        13 array astore concatstringarray 
      }
      { 255 string cvs (; ) 10 2 roll 
        (\string\n)                   % add newline
        11 array astore concatstringarray 
      } ifelse 
    NodeFile exch writestring 
  } if
  NodeType 14 eq {  % dotnode
    5 copy 
    /@@temp ED 
%    gsave  
    @@temp  % to get X Y
    4 -1 roll cvlit pop
    ( OvalNodePos ) (; )  5 2 roll
    20 string cvs (; )   6 2 roll % type
    20 string cvs (; )   7 2 roll %/N@Name
    20 string cvs (; )   8 2 roll % true/false
    Y 20 string cvs (; ) 10 2 roll
    X 20 string cvs (, ) 12 2 roll
    (\string\n)                   % add newline
    13 array astore concatstringarray 
%    grestore
    tx@NodeDict begin NodeFile exch writestring end
  } if
  \fi
  \tx@NewNode
  end 
}%
%
\global\let\psk@name\relax%
\pstree@nodehook%
\global\let\pstree@nodehook\relax}
%
\let\pstree@nodehook\relax
\define@boolkey[psset]{pst-node}[Pst@]{nodealign}[true]{}
\psset[pst-node]{nodealign=false}

\def\pst@nodealign{%
\pst@dimg=\ht\pst@hbox
\advance\pst@dimg-\dp\pst@hbox
\divide\pst@dimg2
\lower\pst@dimg}
%
\def\tx@InitPnode{InitPnode }
\def\pnode{\@ifnextchar[{\pnode@i}{\pnode@iii}}
\def\pnode@i[#1]{\@ifnextchar({\pnode@ii[#1]}{\pnode@ii[#1](0,0)}}
\def\pnode@ii[#1](#2)#3{%
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#2}\pst@tempB%
  \pst@newnode{#3}{10}{\pst@tempA \pst@tempB 3 -1 roll add 3 1 roll add exch }{\tx@InitPnode}%
  \ifPst@showNode\psdot(#3)\uput[\ifx\psk@rot\@empty0\else\psk@rot\fi]{0}(#3){#3}\fi
  \ignorespaces}
%
\def\pnode@iii{\@ifnextchar({\pnode@}{\pnode@(0,0)}}
\def\pnode@(#1)#2{%
  \pst@@getcoor{#1}%
  \pst@newnode{#2}{10}{\pst@coor}{\tx@InitPnode}%
  \ifPst@showNode\psdot(#2)\uput[\ifx\psk@rot\@empty0\else\psk@rot\fi]{0}(#2){#2}\fi
  \ignorespaces}
%
\def\pnodes{\@ifnextchar[{\pnodes@i}{\pnodes@i[0,0]}}
\def\pnodes@i[#1]{\@ifnextchar({\psnodes@ii[#1]}{\pnodes@ii}}
\def\psnodes@ii[#1](#2)#3{%
  \pnode[#1](#2){#3}%
  \@ifnextchar({\psnodes@ii[#1]}{}%
}
%
\def\tx@InitCnode{InitCnode }
%
\def\cnode{\pst@object{cnode}}
\def\cnode@i{\@ifnextchar({\cnode@ii}{\cnode@ii(0,0)}}
\def\cnode@ii(#1)#2#3{%
  \leavevmode
  \hbox{%
    \use@par
    \pst@@getcoor{#1}%
    \pssetlength\pst@dimc{#2}%
    \pst@dimg=\psk@dimen\pslinewidth
    \advance\pst@dimc-\pst@dimg
    \advance\pst@dimc.5\pslinewidth
    \ifPst@nodealign
      \kern\pst@dimc
      \vrule width\z@ height \pst@dimc depth \pst@dimc
    \fi
    \pscircle@do(#1){#2}%
    \pst@newnode{#3}{11}{\pst@coor \pst@number\pst@dimc}{\tx@InitCnode}%
%%    % DG/SR modification begin - Jul. 30, 1997 - Patch 2
%%    %\ifPst@nodealign \kern\pst@dimc\egroup \fi}%
    \ifPst@nodealign\kern\pst@dimc\fi%
%%    % DG/SR modification end
  }%
  \ignorespaces}
%
\def\Cnode{\pst@object{Cnode}}
\def\Cnode@i{\@ifnextchar({\Cnode@ii}{\Cnode@ii(0,0)}}
\def\Cnode@ii(#1)#2{\cnode@ii(#1){\psk@radius}{#2}}%
%
\def\cnodeput{\pst@object{cnodeput}}
\def\cnodeput@i{\@ifnextchar({\cnodeput@iii}{\cnodeput@ii}}
\def\cnodeput@ii#1{%
  \addto@par{rot={#1}}%
  \@ifnextchar({\cnodeput@iii}{\cnodeput@iii(\z@,\z@)}}
\def\cnodeput@iii(#1)#2{%
  \pst@killglue
  \@fixedradiusfalse
  \def\pst@nodehook{\cnodeput@iv{#2}}%
  \pst@makebox{\cput@v{#1}}}
\def\cnodeput@iv#1{%
  \pst@newnode{#1}{11}{\pscirclebox@iv \pst@number\pslinewidth add}{\tx@InitCnode}%
  \global\let\pst@nodehook\relax}
%  
\def\Cnodeput{\pst@object{Cnodeput}}
\def\Cnodeput@i{\@ifnextchar({\Cnodeput@iii}{\Cnodeput@ii}}
\def\Cnodeput@ii#1{%
\addto@par{rot={#1}}%
\@ifnextchar({\Cnodeput@iii}{\Cnodeput@iii(\z@,\z@)}}
\def\Cnodeput@iii(#1)#2{%
\pst@killglue
\@fixedradiustrue
\def\pst@nodehook{\Cnodeput@iv{#2}}%
\pst@makebox{\cput@v{#1}}}
\def\Cnodeput@iv#1{%
\pst@newnode{#1}{11}{%
\pst@number{\wd\pst@hbox} 2 div \pst@number\pst@dima % x y
\pst@number\pst@dimb \pst@number\pslinewidth \psk@dimen .5 sub mul sub }% r
{\tx@InitCnode}%
\global\let\pst@nodehook\relax}
%
\def\circlenode{\pst@object{circlenode}}
\def\circlenode@i#1{\pst@makebox{\circlenode@ii{#1}}}
\def\circlenode@ii#1{%
  \begingroup
  \pst@useboxpar
  \setbox\pst@hbox=\hbox{%
    \cnodeput@iv{#1}%
    \pscirclebox@iii
    \box\pst@hbox}%
  \ifPst@nodealign \psboxseptrue \fi
  \ifpsboxsep \pscirclebox@sep \fi
  \leavevmode
  \ifPst@nodealign\pst@nodealign\fi
  \box\pst@hbox
  \endgroup}
%
\def\Circlenode{\pst@object{Circlenode}}
\def\Circlenode@i#1{\pst@makebox{\Circlenode@ii{#1}}}
\def\Circlenode@ii#1{%
\begingroup
\pst@useboxpar
\pst@dima=\ht\pst@hbox
\advance\pst@dima\dp\pst@hbox
\divide\pst@dima\tw@
\pssetlength\pst@dimb\psk@radius
\setbox\pst@hbox=\hbox{%
\Cnodeput@iv{#1}%
\pscircle(.5\wd\pst@hbox,\pst@dima){\pst@dimb}%
\box\pst@hbox}%
\ifPst@nodealign \psboxseptrue \fi
\ifpsboxsep \psCirclebox@sep \fi
\leavevmode
\ifPst@nodealign\pst@nodealign\fi
\box\pst@hbox
\endgroup}
\def\tx@GetRnodePos{GetRnodePos }
\def\tx@InitRnode{InitRnode }
%
\def\psnode{\pst@object{psnode}}
\def\psnode@i{\@ifnextchar(\psnode@ii{\psnode@ii(0,0)}}
\def\psnode@ii(#1)#2#3{%    #1: coordinates, #2: node name,  #3 contents
  \rput(#1){\rnode{#2}{#3}}}
%
\def\rnode{\@ifnextchar[{\rnode@i}{\def\pst@par{}\rnode@ii}}
\def\rnode@i[#1]{\def\pst@par{ref=#1}\rnode@ii}
\def\rnode@ii#1{\pst@makebox{\rnode@iii\rnode@iv{#1}}}
\def\rnode@iii#1#2{%
% DG modification begin - Jan. 1997
\leavevmode
% DG modification end
\begingroup
% DG/SR modification begin - Apr. 28, 1998 - Patch 6
\pst@useboxpar
% DG/SR modification end
#1%
\if@star\pst@starbox\fi
\ifPst@nodealign\lower\pst@dimb\fi
\hbox{%
\pst@newnode{#2}{16}{%
\pst@number{\ht\pst@hbox}%
\pst@number{\dp\pst@hbox}%
\pst@number{\wd\pst@hbox}%
\pst@number\pst@dima%
\pst@number\pst@dimb}%
{\tx@InitRnode}%
\box\pst@hbox}%
\endgroup}
\def\rnode@iv{%
\pst@dima=\psk@xref\wd\pst@hbox
\ifx\psk@yref\relax
\pst@dimb=\z@
\else
\pst@dimb=\ht\pst@hbox
\advance\pst@dimb\dp\pst@hbox
\pst@dimb=\psk@yref\pst@dimb
\advance\pst@dimb-\dp\pst@hbox
\fi}
%
\define@key[psset]{pst-node}{href}[0]{\pst@checknum{#1}\psk@href}
\psset[pst-node]{href=0}
\define@key[psset]{pst-node}{vref}[0.7ex]{\def\psk@vref{#1}}
\psset[pst-node]{vref=0.7ex}
\def\Rnode{\pst@object{Rnode}}
\def\Rnode@i#1{\pst@makebox{\rnode@iii\Rnode@ii{#1}}}
\def\Rnode@ii{%
% DG modification begin - Jan. 1997
%   - \begingroup removed  as it seems to doesn't work any more
%   - \Rnode doesn't process the optional parameter changes
%\begingroup
\use@par
% DG modification end
\pst@dima=\psk@href\wd\pst@hbox
\advance\pst@dima\wd\pst@hbox
\divide\pst@dima 2
\pssetlength\pst@dimb{\psk@vref}}
\def\tx@DiaNodePos{DiaNodePos }
\def\dianode{\pst@object{dianode}}
\def\dianode@i#1{\pst@makebox{\dianode@ii{#1}}}
\def\dianode@ii#1{%
\begingroup
\pst@useboxpar
\psdiabox@iii
\setbox\pst@hbox=\hbox{%
\pst@newnode{#1}{14}{}{%
/X \pst@number\pst@dima def
/Y \pst@number\pst@dimb def
/w \pst@number\pst@dimc 2 mul def
/h \pst@number\pst@dimd 2 mul def
/NodePos { \tx@DiaNodePos } def}%
\box\pst@hbox}%
\ifPst@nodealign\psboxseptrue\fi
\ifpsboxsep\psdiabox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
\leavevmode
% DG/SR modification end
\ifPst@nodealign\lower\pst@dimb\fi
\box\pst@hbox
\endgroup}
%
\def\tx@TriNodePos{TriNodePos }
\def\tx@InitTriNode{InitTriNode }
%
\def\trinode{\pst@object{trinode}}
\def\trinode@i#1{\pst@makebox{\trinode@ii{#1}}}
\def\trinode@ii#1{%
  \begingroup%
  \pst@useboxpar%
  \pstribox@iii
  \setbox\pst@hbox=\hbox{%
    \pst@newnode{#1}{14}{}{
      \pst@number\pst@dimc
      \pst@number\pst@dimd
      \ifodd\psk@trimode
        exch
        \pst@number\pst@dima
      \else
        \pst@number\pst@dimb
      \fi
      \psk@trimode
      \pst@number{\wd\pst@hbox}
      \pst@number{\ht\pst@hbox}
      \pst@number{\dp\pst@hbox}
      \tx@InitTriNode
    }%
    \box\pst@hbox%
  }%
  \ifPst@nodealign\psboxseptrue\fi
  \ifpsboxsep\pstribox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
  \leavevmode
% DG/SR modification end
  \ifPst@nodealign\lower\pst@tempa\fi
  \box\pst@hbox%
  \endgroup}
%
\def\tx@OvalNodePos{OvalNodePos }
\def\ovalnode{\pst@object{ovalnode}}
\def\ovalnode@i#1{\pst@makebox{\ovalnode@ii{#1}}}
\def\ovalnode@ii#1{%
\begingroup
\pst@useboxpar
\psovalbox@iii
\setbox\pst@hbox=\hbox{%
\pst@newnode{#1}{14}{}{%
/X \pst@number\pst@dima def
/Y \pst@number\pst@dimb def
/w \pst@number\pst@dimc def
/h \pst@number\pst@dimd def
/NodePos { \tx@OvalNodePos } def}%
\unhbox\pst@hbox}%
\ifPst@nodealign\psboxseptrue\fi
\ifpsboxsep\psovalbox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
\leavevmode
% DG/SR modification end
\ifPst@nodealign\lower\pst@dimb\fi
\box\pst@hbox
\endgroup}
%
\def\dotnode{\pst@object{dotnode}}
\def\dotnode@i{\@ifnextchar({\dotnode@ii}{\dotnode@ii(\z@,\z@)}}
\def\dotnode@ii(#1)#2{%
  \leavevmode
  \hbox{%
    \use@par
    \pst@@getcoor{#1}%
    \pst@getdotsize
    \pstree@nodehook
    \ifPst@nodealign
      \pst@dima=\pst@dimg
      \kern\pst@dima
      \vrule width\z@ height \pst@dimh depth \pst@dimh
    \fi
    \pst@newnode{#2}{14}{}{
      \pst@coor
      /Y exch def /X exch def
      /w \pst@number\pst@dimg def
      /h \pst@number\pst@dimh def
      /NodePos { \tx@OvalNodePos } def}%
    \psdot@ii(#1)%
    \ifPst@nodealign\kern\pst@dima\fi}%
  \ifPst@markNode\uput[\ifx\psk@rot\@empty0\else\psk@rot\fi]{0}(#2){#2}\fi
  \ignorespaces}
%
\def\dotnodes{\pst@object{dotnodes}}
\def\dotnodes@i{\use@par\dotnodes@ii}
\def\dotnodes@ii(#1)#2{%
  \dotnode(#1){#2}%
  \@ifnextchar(\dotnodes@ii{\def\pst@par{}}}
%
\define@key[psset]{pst-node}{framesize}{\pst@expandafter\psset@@framesize{#1} \@nil}
\def\psset@@framesize#1 #2\@nil{%
  \pssetlength\pst@dimg{#1}%
  \divide\pst@dimg2
  \edef\psk@framewidth{\pst@number\pst@dimg}%
  \ifx\@empty#2\@empty
    \let\psk@frameheight\psk@framewidth
  \else
    \pssetlength\pst@dimg{#2}%
    \divide\pst@dimg2
    \edef\psk@frameheight{\pst@number\pst@dimg}%
  \fi}
%
\psset[pst-node]{framesize=10pt}
%
\def\fnode{\pst@object{fnode}}
\def\fnode@i{\@ifnextchar({\fnode@ii}{\fnode@ii(\z@,\z@)}}
\def\fnode@ii(#1)#2{%
  \leavevmode
  \pst@killglue
  \hbox{%
    \use@par%
    \begin@ClosedObj%
    \ifPst@nodealign
      \kern\psk@framewidth\p@
      \vrule width\z@ height \psk@frameheight\p@ depth \psk@frameheight\p@
      \edef\pst@coor{0 0 }%
    \else\pst@@getcoor{#1}\fi
    \pst@newnode{#2}{14}{}{
      \pst@coor
      /Y exch def /X exch def
      /d \psk@dimen .5 sub CLW mul neg def
      /r \psk@framewidth d add def
      /l r neg def
      /u \psk@frameheight d add def
      /d u neg def
      /NodePos { \tx@GetRnodePos } def}%
    \addto@pscode{
      /x2 \psk@framewidth CLW \psk@dimen mul sub def
      /y2 \psk@frameheight CLW \psk@dimen mul sub def
      \pst@coor 2 copy
      y2 sub /y1 ED
      x2 sub /x1 exch def
      y2 add /y2 exch def
      x2 add /x2 exch def
      \psk@cornersize
      1 index 0 eq { pop pop \tx@Rect } { \tx@OvalFrame } ifelse}%
    \def\pst@linetype{2}%
    \showpointsfalse%
    \end@ClosedObj%
    \ifPst@nodealign\kern\psk@framewidth\p@\fi}% end of \hbox
  \ignorespaces}
%
%
% This fixes a bug in pst-node, where the XY-direction is wrong
% the types are changed 1<->2 between X<->Y
%
\define@key[psset]{}{XnodesepA}{\pst@getlength{#1}\psk@nodesepA\def\psk@nodeseptypeA{2 }}
\define@key[psset]{}{XnodesepB}{\pst@getlength{#1}\psk@nodesepB\def\psk@nodeseptypeB{2 }}
\define@key[psset]{}{Xnodesep}{%
    \pst@getlength{#1}\psk@nodesepA
    \let\psk@nodesepB\psk@nodesepA
    \def\psk@nodeseptypeA{2 }%
    \def\psk@nodeseptypeB{2 }}
\define@key[psset]{}{YnodesepA}{\pst@getlength{#1}\psk@nodesepA\def\psk@nodeseptypeA{1 }}
\define@key[psset]{}{YnodesepB}{\pst@getlength{#1}\psk@nodesepB\def\psk@nodeseptypeB{1 }}
\define@key[psset]{}{Ynodesep}{%
    \pst@getlength{#1}\psk@nodesepA
    \let\psk@nodesepB\psk@nodesepA
    \def\psk@nodeseptypeA{1 }%
    \def\psk@nodeseptypeB{1 }}
%%%% end bugfix %%%%%
\define@key[psset]{pst-node}{nodesepA}[0pt]{\pst@getlength{#1}\psk@nodesepA \def\psk@nodeseptypeA{0 }}
\define@key[psset]{pst-node}{nodesepB}[0pt]{\pst@getlength{#1}\psk@nodesepB \def\psk@nodeseptypeB{0 }}
\define@key[psset]{pst-node}{nodesep}[0pt]{%
  \pst@getlength{#1}\psk@nodesepA
  \let\psk@nodesepB\psk@nodesepA
  \def\psk@nodeseptypeA{0 }%
  \def\psk@nodeseptypeB{0 }}
\psset[pst-node]{nodesep=0pt}
%\define@key[psset]{pst-node}{XnodesepA}[]{\pst@getlength{#1}\psk@nodesepA \def\psk@nodeseptypeA{1 }}
%\define@key[psset]{pst-node}{XnodesepB}[]{\pst@getlength{#1}\psk@nodesepB \def\psk@nodeseptypeB{1 }}
%\define@key[psset]{pst-node}{Xnodesep}[]{%
%  \pst@getlength{#1}\psk@nodesepA
%  \let\psk@nodesepB\psk@nodesepA
%  \def\psk@nodeseptypeA{1 }%
%  \def\psk@nodeseptypeB{1 }}
%\define@key[psset]{pst-node}{YnodesepA}[]{\pst@getlength{#1}\psk@nodesepA \def\psk@nodeseptypeA{2 }}
%\define@key[psset]{pst-node}{YnodesepB}[]{\pst@getlength{#1}\psk@nodesepB \def\psk@nodeseptypeB{2 }}
%\define@key[psset]{pst-node}{Ynodesep}[]{
%  \pst@getlength{#1}\psk@nodesepA
%  \let\psk@nodesepB\psk@nodesepA
%  \def\psk@nodeseptypeA{2 }%
%  \def\psk@nodeseptypeB{2 }}
\define@key[psset]{pst-node}{armA}[10pt]{\pst@getlength{#1}\psk@armA \def\psk@armtypeA{0 }}
\define@key[psset]{pst-node}{armB}[10pt]{\pst@getlength{#1}\psk@armB \def\psk@armtypeB{0 }}
\define@key[psset]{pst-node}{arm}[10pt]{%
  \pst@getlength{#1}\psk@armA
  \let\psk@armB\psk@armA
  \def\psk@armtypeA{0 }%
  \def\psk@armtypeB{0 }}
\psset[pst-node]{arm=10pt}
\define@key[psset]{pst-node}{XarmA}[]{\pst@getlength{#1}\psk@armA \def\psk@armtypeA{1 }}
\define@key[psset]{pst-node}{XarmB}[]{\pst@getlength{#1}\psk@armB \def\psk@armtypeB{1 }}
\define@key[psset]{pst-node}{Xarm}{%
  \pst@getlength{#1}\psk@armA
  \let\psk@armB\psk@armA
  \def\psk@armtypeA{1 }%
  \def\psk@armtypeB{1 }}
\define@key[psset]{pst-node}{YarmA}[]{\pst@getlength{#1}\psk@armA \def\psk@armtypeA{2 }}
\define@key[psset]{pst-node}{YarmB}[]{\pst@getlength{#1}\psk@armB \def\psk@armtypeB{2 }}
\define@key[psset]{pst-node}{Yarm}[]{%
  \pst@getlength{#1}\psk@armA
  \let\psk@armB\psk@armA
  \def\psk@armtypeA{2 }%
  \def\psk@armtypeB{2 }}
\define@key[psset]{pst-node}{offsetA}[0pt]{\pst@getlength{#1}\psk@offsetA}
\define@key[psset]{pst-node}{offsetB}[0pt]{\pst@getlength{#1}\psk@offsetB}
\define@key[psset]{pst-node}{offset}[0pt]{\pst@getlength{#1}\psk@offsetA\let\psk@offsetB\psk@offsetA}
\psset[pst-node]{offset=0pt}
\define@key[psset]{pst-node}{angleA}[0]{\pst@getangle{#1}\psk@angleA}
\define@key[psset]{pst-node}{angleB}[0]{\pst@getangle{#1}\psk@angleB}%
\define@key[psset]{pst-node}{angle}[0]{%
  \pst@getangle{#1}\psk@angleA
  \let\psk@angleB\psk@angleA}
\psset[pst-node]{angle=0}
\define@key[psset]{pst-node}{arcangleA}[8]{\pst@getangle{#1}\psk@arcangleA}
\define@key[psset]{pst-node}{arcangleB}[8]{\pst@getangle{#1}\psk@arcangleB}%
\define@key[psset]{pst-node}{arcangle}[8]{%
  \pst@getangle{#1}\psk@arcangleA
  \let\psk@arcangleB\psk@arcangleA}
\psset[pst-node]{arcangle=8}
\define@key[psset]{pst-node}{ncurvA}[0.67]{\pst@checknum{#1}\psk@ncurvA}
\define@key[psset]{pst-node}{ncurvB}[0.67]{\pst@checknum{#1}\psk@ncurvB}%
\define@key[psset]{pst-node}{ncurv}[0.67]{\pst@checknum{#1}\psk@ncurvA\let\psk@ncurvB\psk@ncurvA}
\psset[pst-node]{ncurv=0.67}
%
\def\tx@GetCenter{GetCenter }
\def\tx@XYPos{XYPos }
\def\tx@GetEdge{GetEdge }
\def\tx@AddOffset{AddOffset }
\def\tx@GetEdgeA{GetEdgeA }
\def\tx@GetEdgeB{GetEdgeB }
\def\tx@GetArmA{GetArmA }
\def\tx@GetArmB{GetArmB }
%
\def\check@arrow#1#2{%
  \check@@arrow#2-\@nil
  \if@pst\addto@par{arrows=#2}\def\next{#1}%
  \else\def\next{#1{#2}}\fi
  \next}
\def\check@@arrow#1-#2\@nil{%
\ifx\@nil#2\@nil\@pstfalse\else\@psttrue\fi}
%
\def\tx@InitNC{InitNC }
\def\nc@object#1#2#3#4#5{%
  \csname begin@#1Obj\endcsname
  \showpointsfalse
  \pst@getnode{#2}\pst@tempa
  \pst@getnode{#3}\pst@tempb
  \gdef\npos@default{#4 }%
  \addto@pscode{%
    /NCLW CLW def
    \pst@nodedict
    \psk@offsetA
    \psk@offsetB neg
    \psk@nodesepA
    \psk@nodesepB
    \psk@nodeseptypeA
    \psk@nodeseptypeB
    \pst@tempa
    \pst@tempb
    \tx@InitNC { #5 } if
    end }%
  \def\use@pscode{%
    \pst@Verb{gsave \tx@STV newpath \pst@code\space grestore}%
    \gdef\pst@code{}}%
  \csname end@#1Obj\endcsname
  \pst@shortput}
%
\def\npos@default{.5 }
%
\def\pc@object#1{%
  \@ifnextchar({\pc@@object#1}{\pst@getarrows{\pc@@object#1}}}
\def\pc@@object#1(#2)(#3){%
  \pnode(#2){@@A}\pnode(#3){@@B}%
  #1{@@A}{@@B}}
%
\def\tx@LPutLine{LPutLine }
\def\tx@LPutLines{LPutLines }
\def\tx@BezierMidpoint{BezierMidpoint }
\def\tx@HPosBegin{HPosBegin }
\def\tx@HPosEnd{HPosEnd }
\def\tx@HPutLine{HPutLine }
\def\tx@HPutLines{HPutLines }
\def\tx@VPosBegin{VPosBegin }
\def\tx@VPosEnd{VPosEnd }
\def\tx@VPutLine{VPutLine }
\def\tx@VPutLines{VPutLines }
\def\tx@HPutCurve{HPutCurve }
\def\tx@NCCoor{NCCoor }
\def\tx@NCLine{NCLine }
%
\def\ncline{\pst@object{ncline}}
\def\ncline@i{\check@arrow{\ncline@ii}}
\def\ncline@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{\tx@NCLine}}
%
\def\pcline{\pst@object{pcline}}
\def\pcline@i{\pc@object\ncline@ii}
%
\def\ncLine{\pst@object{ncLine}}
\def\ncLine@i{\check@arrow{\ncLine@ii}}
\def\ncLine@ii#1#2{\nc@object{Open}{#1}{#2}{.5}%
% DG/SR modification begin - Apr. 14, 1999 - Patch 9
%{\tx@NCLine /LPutPos { xB xA yB yA \tx@LPutLine } def}}
{\tx@NCLine /LPutPos { xB yB xA yA \tx@LPutLine } def}}
% DG/SR modification end
%
\def\tx@NCLines{NCLines }
\def\nclines{\pst@object{nclines}}
\def\nclines@i{\check@arrow\nclines@ii}
\def\nclines@ii#1#2{%
\begingroup
\use@par
\def\pst@aftercoors{\nclines@iii{#1}{#2}}%
\def\pst@coors{}%
\pst@@getcoors}
\def\nclines@iii#1#2{%
\nc@object{Open}{#1}{#2}{.5}{%
tx@Dict begin \psline@iii pop end
mark \pst@coors \tx@NCLines}%
\endgroup
\ignorespaces}
\def\tx@NCCurve{NCCurve }
\def\nccurve{\pst@object{nccurve}}
\def\nccurve@i{\check@arrow{\nccurve@ii}}
\def\nccurve@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
  /AngleA \psk@angleA\space def /AngleB \psk@angleB\space def
  \psk@ncurvB\space \psk@ncurvA\space
  \tx@NCCurve}}
\def\pccurve{\pst@object{pccurve}}
\def\pccurve@i{\pc@object\nccurve@ii}
%
\def\ncarc{\pst@object{ncarc}}
\def\ncarc@i{\check@arrow{\ncarc@ii}}
\def\ncarc@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
  yB yA sub xB xA sub \tx@Atan dup
  \psk@arcangleA\space add /AngleA exch def
  \psk@arcangleB\space sub 180 add /AngleB exch def
  \psk@ncurvB\space \psk@ncurvA\space
  \tx@NCCurve}}
\def\pcarc{\pst@object{pcarc}}
\def\pcarc@i{\pc@object\ncarc@ii}
%
\def\tx@NCAngles{NCAngles }
%
%border or center as reference point (hv)
\define@boolkey[psset]{pst-node}[Pst@]{pcRef}[true]{}
\psset[pst-node]{pcRef=false}
%
\def\ncangles{\pst@object{ncangles}}
\def\ncangles@i{\check@arrow{\ncangles@ii}}
\def\ncangles@ii#1#2{%
  \nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \tx@NCAngles}}
\def\ncangles@iii{
  tx@Dict begin \psline@iii pop end
  /AngleA \psk@angleA def
  /AngleB \psk@angleB def
  /ArmA \psk@armA \ifPst@pcRef 
    GetEdgeA yA yA1 sub dup mul xA xA1 sub dup mul add sqrt sub \fi def
  /ArmB \psk@armB def
  /ArmTypeA \psk@armtypeA def
  /ArmTypeB \psk@armtypeB def }
%
\def\pcangles{\pst@object{pcangles}}
\def\pcangles@i{\pc@object\ncangles@ii}
\def\tx@NCAngle{NCAngle }
\def\ncangle{\pst@object{ncangle}}
\def\ncangle@i{\check@arrow{\ncangle@ii}}
\def\ncangle@ii#1#2{%
\nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \tx@NCAngle}}
\def\pcangle{\pst@object{pcangle}}
\def\pcangle@i{\pc@object\ncangle@ii}
\def\tx@NCBar{NCBar }
\def\ncbar{\pst@object{ncbar}}
\def\ncbar@i{\check@arrow{\ncbar@ii}}
\def\ncbar@ii#1#2{\nc@object{Open}{#1}{#2}{1.5}{%
\ncangles@iii /AngleB \psk@angleA def \tx@NCBar}}
\def\pcbar{\pst@object{pcbar}}
\def\pcbar@i{\pc@object\ncbar@ii}
%
\define@key[psset]{pst-node}{lineAngle}[0]{%
  \ifdim#1pt=\z@\else\psset{armB=0.5}\fi
  \def\psk@lineAngle{#1}}%
\psset[pst-node]{lineAngle=0}%
%
\def\tx@NCDiag{NCDiag }
\def\ncdiag{\pst@object{ncdiag}}
\def\ncdiag@i{\check@arrow{\ncdiag@ii}}
\def\ncdiag@ii#1#2{%
  \nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \psk@lineAngle\space \tx@NCDiag}}
%
\def\pcdiag{\pst@object{pcdiag}}
\def\pcdiag@i{\pc@object\ncdiag@ii}
%
\def\tx@NCDiagg{NCDiagg }
\def\ncdiagg{\pst@object{ncdiagg}}
\def\ncdiagg@i{\check@arrow{\ncdiagg@ii}}
\def\ncdiagg@ii#1#2{%
  \nc@object{Open}{#1}{#2}{.5}{\ncangles@iii \psk@lineAngle\space \tx@NCDiagg}}
\def\pcdiagg{\pst@object{pcdiagg}}
%
\def\pcdiagg@i{\pc@object\ncdiagg@ii}
\def\tx@NCLoop{NCLoop }
\define@key[psset]{pst-node}{loopsize}{\pst@getlength{#1}\psk@loopsize}
\psset[pst-node]{loopsize=1cm}
\def\ncloop{\pst@object{ncloop}}
\def\ncloop@i{\check@arrow{\ncloop@ii}}
\def\ncloop@ii#1#2{%
\nc@object{Open}{#1}{#2}{2.5}%
{\ncangles@iii /loopsize \psk@loopsize def \tx@NCLoop}}
\def\pcloop{\pst@object{pcloop}}
\def\pcloop@i{\pc@object\ncloop@ii}
\def\tx@NCCircle{NCCircle }
\def\nccircle{\pst@object{nccircle}}
\def\nccircle@i{\check@arrow{\nccircle@ii}}
\def\nccircle@ii#1#2{%
\pssetlength\pst@dima{#2}%
\nc@object{Open}{#1}{#1}{.5}{%
/AngleA \psk@angleA def
/r \pst@number\pst@dima def
\tx@NCCircle \psarc@v end}}
\def\tx@NCBox{NCBox }
\def\ncbox{\pst@object{ncbox}}
\def\ncbox@i{\check@arrow{\ncbox@ii}}
\def\ncbox@ii#1#2{%
\def\pst@linetype{2}%
\nc@object{Closed}{#1}{#2}{.5}{%
tx@Dict begin \psline@iii pop end
\psk@boxheight \psk@boxdepth
\tx@NCBox}}
\def\pcbox{\pst@object{pcbox}}
\def\pcbox@i{\pc@object\ncbox@ii}
\def\tx@NCArcBox{NCArcBox }
\define@key[psset]{pst-node}{boxheight}[0.4cm]{\pst@getlength{#1}\psk@boxheight}
\define@key[psset]{pst-node}{boxdepth}[0.4cm]{\pst@getlength{#1}\psk@boxdepth}
\define@key[psset]{pst-node}{boxsize}[0.4cm]{%
  \pst@getlength{#1}\psk@boxheight%  
  \let\psk@boxdepth\psk@boxheight}
\psset[pst-node]{boxsize=0.4cm}
%
\def\ncarcbox{\pst@object{ncarcbox}}
\def\ncarcbox@i{\check@arrow{\ncarcbox@ii}}
\def\ncarcbox@ii#1#2{%
\def\pst@linetype{1}%
\nc@object{Closed}{#1}{#2}{.5}{%
\psk@arcangleA \psk@boxheight \psk@boxdepth \pst@number\pslinearc
\tx@NCArcBox}}
\def\pcarcbox{\pst@object{pcarcbox}}
\def\pcarcbox@i{\pc@object\ncarcbox@ii}
\def\tx@Tfan{Tfan }
% Changed according pst-beta.bug December 3, 1993
% nrot=:<angle> does not work when : is active.
\begingroup
\catcode`\:=13
\gdef\pst@activerot{\def:{\string:}}
\endgroup
\define@key[psset]{pst-node}{nrot}[0]{%
  \begingroup
  \pst@activerot
  \pst@expandafter{\@ifnextchar:{\psset@@nrot}{\psset@@rot}}{#1}\@nil
  \global\let\pst@tempg\psk@rot
  \endgroup
  \let\psk@nrot\pst@tempg}
%  
\def\psset@@nrot:#1\@nil{%
  \psset@@rot#1\@nil
  \edef\psk@rot{NAngle \ifx\psk@rot\@empty\else\psk@rot add \fi}}
\psset[pst-node]{nrot=0}
%
\def\tx@LPutCoor{LPutCoor }
\def\tx@LPut{LPut }
\define@key[psset]{pst-node}{npos}[{}]{%
  \def\pst@tempa{#1}%
  \ifx\pst@tempa\@empty\def\psk@npos{\npos@default}\else\pst@checknum{#1}\psk@npos\fi}
\psset[pst-node]{npos=}
%
\def\ncput{\pst@object{ncput}}
\def\ncput@i{\pst@killglue\pst@makebox{\ncput@ii}}
\def\ncput@ii{%
  \begingroup%
  \use@par%
  \if@star\pst@starbox\fi%
  \pst@makesmall\pst@hbox%
  \pst@rotate\psk@nrot\pst@hbox%
  \ncput@iii%
  \endgroup%
  \pst@shortput}
\def\ncput@iii{%
  \leavevmode%
  \hbox{%
    \pst@Verb{
      \pst@nodedict
      /t \psk@npos def
      \tx@LPut
      end
      \tx@PutBegin}%
    \box\pst@hbox%
    \pst@Verb{\tx@PutEnd}}}
%
\def\naput{\pst@object{naput}}
\def\naput@i{\pst@killglue\pst@makebox{\naput@ii{NAngle 90 add}}}
\def\naput@ii#1{%
  \begingroup
%  \addto@par{labelsep=15pt}%
  \use@par
  \if@star\pst@starbox\fi
  \def\psk@refangle{#1 }%
  \let\psk@rot\psk@nrot
  \pst@Verb{ 
    gsave  STV CP T /ps@refangle {#1 } def 
    /ps@rot { \psk@rot } def grestore }%ADDED (MJS)
  \uput@vii
  {exch pop add a \tx@PtoC h1 add exch w1 add exch }%
  {tx@Dict /NCLW known { NCLW add } if }%
  \ncput@iii
  \endgroup
  \pst@shortput}
%
\def\nbput{\pst@object{nbput}}
\def\nbput@i{\pst@killglue\pst@makebox{\naput@ii{NAngle 90 sub}}}
\define@key[psset]{pst-node}{tpos}[0.5]{%
  \pst@checknum{#1}\psk@tpos
  \ifdim\psk@tpos \p@<\z@
    \def\psk@tpos{.5}%
% DG/SR modification begin - Sep. 23, 1998 - Patch 7
%\@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@epha
    \@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@ehpa
% DG/SR modification end
  \else
    \ifdim\psk@tpos \p@>\p@
      \def\psk@tpos{.5}%
% DG/SR modification begin - Sep. 23, 1998 - Patch 7
%\@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@epha
      \@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@ehpa%
% DG/SR modification end
    \fi%
  \fi}
\psset[pst-node]{tpos=0.5}
%
\def\nlput{\pst@object{nlput}}
\def\nlput@i(#1)(#2)#3#4{%
  \begin@SpecialObj
  \psLDNode(#1)(#2){#3}{temp@lnput}
  \pcline[linestyle=none](#1)(temp@lnput)%
  \ncput[npos=1]{#4}%
  \end@SpecialObj}
%
\def\tvput{\pst@object{tvput}}
\def\tvput@i{\pst@makebox{\psput@tput{H}{1}}}
\def\tlput{\pst@object{tlput}}
\def\tlput@i{\pst@makebox{\psput@tput{H}{true}}}
\def\trput{\pst@object{trput}}
\def\trput@i{\pst@makebox{\psput@tput{H}{false}}}
\def\thput{\pst@object{thput}}
\def\thput@i{\pst@makebox{\psput@tput{V}{1}}}
\def\taput{\pst@object{taput}}
\def\taput@i{\pst@makebox{\psput@tput{V}{true}}}
\def\tbput{\pst@object{tbput}}
\def\tbput@i{\pst@makebox{\psput@tput{V}{false}}}
\def\tx@HPutAdjust{HPutAdjust }
\def\tx@VPutAdjust{VPutAdjust }
\def\psput@tput#1#2{%
  \begingroup
  \use@par
  \pst@tputmakesmall
  \leavevmode
  \hbox{%
    \pst@Verb{%
      \pst@nodedict
      /t \psk@tpos \pst@tposflip def
      tx@NodeDict /HPutPos known
        { #1PutPos }
        { CP /Y exch def /X exch def /NAngle 0 def /NCLW 0 def }
      ifelse
      /Sin NAngle sin def
      /Cos NAngle cos def
      /s \pst@number\pslabelsep NCLW add def
      /l \pst@number\pst@dima def
      /r \pst@number\pst@dimb def
      /h \pst@number\pst@dimc def
      /d \pst@number\pst@dimd def
% DG/SR modification begin - Sep. 26, 1997 - Patch 4
%\ifnum1=0#2\else
      \ifnum1=0#2 \else
% DG/SR modification end
        /flag #2 def
        \csname tx@#1PutAdjust\endcsname
      \fi
      \tx@LPutCoor
      end
      \tx@PutBegin}%
    \box\pst@hbox
    \pst@Verb{\tx@PutEnd}}%
  \endgroup
  \pst@shortput}
%  
\def\pst@tposflip{}
\def\pst@tputmakesmall{%
%
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\pst@dimg=\psk@href\pst@dimg
\pst@dimb\pst@dima
\advance\pst@dima\pst@dimg % leftsize
\advance\pst@dimb-\pst@dimg % rightsize
\pst@dimd=\psk@vref\relax
\pst@dimc=\ht\pst@hbox
\advance\pst@dimc-\pst@dimd % height
\advance\pst@dimd\dp\pst@hbox % depth
\setbox\pst@hbox=\hbox to\z@{%
\kern-\pst@dima\vbox to\z@{\vss\box\pst@hbox\vskip-\pst@dimd}\hss}}
\def\MakeShortNab#1#2{%
  \def\pst@shortput@nab{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \let\pst@tempg\naput
    \else
      \ifx#2\next
        \let\pst@tempg\nbput
      \else
        \ifx\@sptoken\next
          \let\pst@tempg\pst@shortput
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortNab{^}{_}
\def\MakeShortTablr#1#2#3#4{%
  \def\pst@shortput@tablr{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \let\pst@tempg\taput
    \else
      \ifx#2\next
        \let\pst@tempg\tbput
      \else
        \ifx#3\next
          \let\pst@tempg\tlput
        \else
          \ifx#4\next
            \let\pst@tempg\trput
          \else
            \ifx\@sptoken\next
              \let\pst@tempg\pst@shortput
            \fi
          \fi
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortTablr{^}{_}{<}{>}
\def\MakeShortTab#1#2{%
  \def\pst@shortput@tab{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \def\pst@tempg{%
        \@nameuse{%
          t\ifodd\psk@treemode\ifpstreeflip b\else a\fi
          \else\ifpstreeflip r\else l\fi\fi put}}%
    \else
      \ifx#2\next
        \def\pst@tempg{%
          \@nameuse{%
            t\ifodd\psk@treemode\ifpstreeflip a\else b\fi
            \else\ifpstreeflip l\else r\fi\fi put}}%
      \else
        \ifx\@sptoken\next
          \let\pst@tempg\pst@shortput
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortTab{^}{_}
\define@key[psset]{pst-node}{shortput}[none]{%
  \def\pst@tempg{#1}%
  \ifx\pst@tempg\@none
    \let\pst@shortput\ignorespaces
  \else
    \@ifundefined{pst@shortput@#1}%
     {\@pstrickserr{Bad short put: `#1'}\@ehpa}%
     {\edef\pst@shortput{\noexpand\afterassignment\expandafter\noexpand
      \csname pst@shortput@#1\endcsname\noexpand\let\noexpand\next}}%
  \fi}
\psset[pst-node]{shortput=none}
%
\def\lput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\lput@i}{\lput@ii}}}
\def\lput@i[#1]{\addto@par{ref=#1}\lput@ii}
\def\lput@ii{\@ifnextchar({\lput@iv}{\lput@iii}}
\def\lput@iii#1{\addto@par{nrot=#1}\@ifnextchar({\lput@iv}{\ncput@i}}
\def\lput@iv(#1){\addto@par{npos=#1}\ncput@i}
\def\mput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\mput@i}{\ncput@i}}}
\def\mput@i[#1]{\addto@par{ref=#1}\ncput@i}
\def\Lput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Lput@ii}{\Lput@i}}}
\def\Lput@i#1{\addto@par{labelsep=#1}\Lput@ii}
\def\Lput@ii[#1]{\addto@par{ref={#1}}\@ifnextchar({\Lput@iv}{\Lput@iii}}
\def\Lput@iii#1{\addto@par{nrot={#1}}\@ifnextchar({\Lput@iv}{\Lput@v}}
\def\Lput@iv(#1){\addto@par{npos=#1}\Lput@v}
\def\Lput@v{\pst@killglue\pst@makebox{\Lput@vi}}
\def\Lput@vi{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\Rput@vi
\pst@makesmall\pst@hbox
\ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%\pst@rotate\psk@nrot\pst@hbox
\ncput@iii
\endgroup
\pst@shortput}
\def\Mput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Mput@ii}{\Mput@i}}}
\def\Mput@i#1{\addto@par{labelsep=#1}\Mput@ii}
\def\Mput@ii[#1]{\addto@par{ref={#1}}\Lput@v}
\def\aput@#1{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\aput@i#1}{\aput@ii#1}}}
\def\aput@i#1[#2]{\addto@par{labelsep=#2}\aput@ii#1}
\def\aput@ii#1{\@ifnextchar({\aput@iv#1}{\aput@iii#1}}
\def\aput@iii#1#2{\addto@par{nrot=#2}\@ifnextchar({\aput@iv#1}{#1}}
\def\aput@iv#1(#2){\addto@par{npos=#2}#1}
\def\aput{\aput@\naput@i}
\def\bput{\aput@\nbput@i}
\def\Aput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Aput@i}{\naput@i}}}
\def\Aput@i[#1]{\addto@par{labelsep=#1}\naput@i}
\def\Bput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Bput@i}{\nbput@i}}}
\def\Bput@i[#1]{\addto@par{labelsep=#1}\nbput@i}
%
\def\node@coor#1;#2\@nil{%  for normal nodes (name)
  \pst@getnode{#1}\pst@tempg
  \edef\pst@coor{%
    \pst@nodedict
    tx@NodeDict \pst@tempg known
    \pslbrace \pst@tempg load \tx@GetCenter \psrbrace
    \pslbrace 0 0 \psrbrace ifelse
    end }}
%
\def\Node@coor[#1]#2;#3\@nil{%  for special nodes ([...]{node}node)
\begingroup
\psset{angle=0,#1}%   angle=0, to prevent problems if angle is set globally
\@ifnextchar\bgroup{\Node@@@coor}% we have an additional node [...]{node}
                   {\Node@@coor}#2\@nil% we have  [...]node
\endgroup
\let\pst@coor\pst@tempg}
%
\def\Node@@coor#1\@nil{%
\pst@getnode{#1}\pst@tempg
\xdef\pst@tempg{%
\pst@nodedict
tx@NodeDict \pst@tempg known
  { \psk@nodesepA \psk@angleA 
    \pst@tempg load \psk@nodeseptypeA \tx@GetEdge
    \psk@offsetA \psk@angleA \tx@AddOffset
    \pst@tempg load \tx@GetCenter
    3 -1 roll add 3 1 roll add exch }
  { CP } ifelse end }}
%
\def\Node@@@coor#1{%   [...]{#1}node
\pst@@getcoor{#1}%
\def\psk@angleA{%
  \pst@tempg load \tx@GetCenter \pst@coor
  3 -1 roll sub 3 1 roll sub neg \tx@Atan \psk@angleB add
  }%
\Node@@coor}
%
\def\nput{\pst@object{nput}}
\def\nput@i#1#2{\pst@killglue\pst@makebox{\nput@ii{#1}{#2}}}
\def\nput@ii#1#2{%
  \begingroup
  \use@par
  \if@star\pst@starbox\fi%
  \psset[pstricks]{refangle=#1}%
  \let\psk@angleA\psk@refangle
  \edef\psk@nodesepA{\pst@number\pslabelsep}%
  \def\psk@nodeseptypeA{0 }%
  \pslabelsep\z@
  \uput@vi
  \Node@@coor#2\@nil
  \let\pst@coor\pst@tempg
  \leavevmode
  \psput@special\pst@hbox
  \endgroup
  \ignorespaces}
%  
\newcount\psrow
\newcount\pscol
\newcount\psmatrixcnt
\newskip\psrowsep
\newskip\pscolsep
%
\define@key[psset]{pst-node}{colsep}[1.5cm]{\pssetlength\pscolsep{#1}}
\define@key[psset]{pst-node}{rowsep}[1.5cm]{\pssetlength\psrowsep{#1}}
\psset[pst-node]{colsep=1.5cm}
\psset[pst-node]{rowsep=1.5cm}
\newif\ifpsmatrix
% DG/SR modification begin - Nov. 27, 1998 - Patch 8
%\let\mscount\@multicnt
\ifx\mscount\@undefined\let\mscount\@multicnt\fi
% DG/SR modification end
\def\psmatrix{\begingroup{\ifnum0=`}\fi % Don't want to expand any &.
  \@ifnextchar[{\psmatrix@i}{\ifnum0=`{\fi}{}\psmatrix@ii}}
\def\psmatrix@i[#1]{%
  \ifnum0=`{\fi}{}%
  \psset{#1}%
  \psmatrix@ii}
\def\psmatrix@ii{%
  \KillGlue
  \edef\psm@beginmath{%
    \ifmmode$\m@th\ifinner\textstyle\else\displaystyle\fi\fi}%
  \edef\psm@endmath{\ifmmode$\fi}%
  \let\\\psm@cr
  \advance\psmatrixcnt by \@ne
  \def\psm@thenode{M-\the\psmatrixcnt-\the\psrow-\the\pscol}%
  \tabskip\z@
  \psrow=\@ne
  \pscol\z@
  \psset{shortput=tablr}%
  \leavevmode
  \vbox\bgroup\halign\bgroup&%
  \begingroup
  \global\advance\pscol by \@ne
  \csname psrowhook\romannumeral\psrow\endcsname
  \csname pscolhook\romannumeral\pscol\endcsname
  \psm@beginnode##\psm@endnode\endgroup
  \cr}
%
\def\endpsmatrix{%
  \crcr\egroup\unskip\egroup
  \endgroup}
%
% hv 2007-10-16  fix bug with \\[name=...]
%\def\psm@cr{{\ifnum0=`}\fi\@ifnextchar[{\psm@@cr}{\psm@@@cr{}}}
\def\psm@cr{{\ifnum0=`}\fi\ps@ifnextchar[{\psm@@cr}{\psm@@@cr{}}}
%
\def\psm@@cr[#1]{\psm@@@cr{\vskip#1\relax}}
\def\psm@@@cr#1{%
  \ifnum0=`{\fi}{}\cr
  \noalign{%
  \global\advance\psrow 1
  \global\pscol\z@
  \vskip\psrowsep
  #1}}
\def\psm@beginnode{%
  \@ifnextchar\psm@endnode
    {\let\psm@endnode@i\relax\setbox\pst@hbox=\hbox{}}%
    {\pst@object{psm@beginnode}}}
\def\psm@beginnode@i{%
  \setbox\pst@hbox=\hbox\bgroup
  \psm@beginmath
  \begingroup
  \ignorespaces}
\def\psm@endnode@i{%
  \unskip
  \endgroup
  \psm@endmath
  \egroup
  \use@par
  \@psttrue}
\def\psm@endnode{%
  \@pstfalse
  \psm@endnode@i
  \ifnum\pscol>1\relax \pshskip\pscolsep \fi
  \psk@mnodesize
  \hfil
  \Pst@nodealigntrue
  \if@pst\csname mnode@\psk@mnode\endcsname
  \else\csname mnode@\psk@emnode\endcsname\fi
  \psk@mcol
  \psk@@mnodesize}
% DG/SR modification begin - Sep. 3, 1999 - Patch 10 - From Michael Sharpe
%\def\psspan#1{\mscount#1\relax\loop\ifnum\mscount>\@ne \sp@n\repeat}
\def\psspan#1{\global\mscount#1\relax\pstloop\ifnum\mscount>\@ne\sp@n\repeat}
\def\pstloop#1\repeat{\gdef\pstiterate{#1\relax\expandafter\pstiterate\fi}%
  \pstiterate
  \let\pstiterate\relax}
% DG/SR modification end
\define@key[psset]{pst-node}{name}[\relax]{\pst@getnode{#1}\psk@name}
\let\psk@name\relax
\define@key[psset]{pst-node}{mcol}[c]{%
  \ifx r#1\relax\let\psk@mcol\relax\else
    \ifx l#1\relax\let\psk@mcol\hfill\else
    \let\psk@mcol\hfil\fi\fi}
\psset[pst-node]{mcol=c}
%
\define@key[psset]{pst-node}{mnodesize}[-1pt]{%
  \pssetlength\pst@dimg{#1}%
  \ifdim\pst@dimg<\z@
    \let\psk@mnodesize\relax
    \let\psk@@mnodesize\relax
  \else
    \edef\psk@mnodesize{\noexpand\hbox to\number\pst@dimg sp\noexpand\bgroup}%
    \let\psk@@mnodesize\egroup
  \fi}
\psset[pst-node]{mnodesize=-1pt}
%
\def\mnode@R{\rnode@iii\Rnode@ii{\psm@thenode}}
\def\mnode@r{\rnode@iii\rnode@iv{\psm@thenode}}
\def\mnode@oval{\ovalnode@ii{\psm@thenode}}
\def\mnode@tri{\trinode@ii{\psm@thenode}}
\def\mnode@dia{\dianode@ii{\psm@thenode}}
\def\mnode@C{{\Pst@nodealigntrue\cnode@ii(\z@,\z@){\psk@radius}{\psm@thenode}}}
\def\mnode@f{{\Pst@nodealigntrue\fnode@ii(\z@,\z@){\psm@thenode}}}
\def\mnode@circle{\circlenode@ii{\psm@thenode}}
% hv modification begin - Aug. 16, 2007
\def\mnode@Circle{\Circlenode@ii{\psm@thenode}}
% hv modification end - Aug. 16, 2007
\def\mnode@p{\pnode(\z@,\z@){\psm@thenode}}
% DG/SR modification begin - Jul. 22, 1997 - Patch 1
\def\mnode@dot{\dotnode@ii(\z@,\z@){\psm@thenode}}
% DG/SR modification end
\def\mnode@none{\box\pst@hbox}
%
\define@key[psset]{pst-node}{mnode}[R]{%
  \@ifundefined{mnode@#1}%
    {\@pstrickserr{\string\psmatrix\space node `#1' not defined.}\@ehpa}%
    {\edef\psk@mnode{#1}}}
\define@key[psset]{pst-node}{emnode}[none]{%
  \@ifundefined{mnode@#1}%
    {\@pstrickserr{\string\psmatrix\space node `#1' not defined.}\@ehpa}%
    {\edef\psk@emnode{#1}}}
\psset[pst-node]{mnode=R,emnode=none}
%
%%%% FROM pst-coil.tex
\def\nccoil{\pst@object{nccoil}}
\def\nccoil@i{\check@arrow{\nccoil@ii}}
\def\nccoil@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{
  \tx@NCCoor
  tx@Dict begin
  4 2 roll
  \psk@coilwidth \pscoilheight
  \psk@coilarmA \psk@coilarmB
  \psk@coilaspect \psk@coilinc
  \pst@coildict \tx@Coil end
  end}%
}
\def\nczigzag{\pst@object{nczigzag}}
\def\nczigzag@i{\check@arrow{\nczigzag@ii}}
\def\nczigzag@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{
  \tx@NCCoor
  tx@Dict begin
  4 2 roll
  \pscoilheight
  \psk@coilwidth
  \psk@coilarmA
  \psk@coilarmB
  \pst@coildict \tx@ZigZag end
  \psline@iii
  \tx@Line
  end}%
}
% \psGetNodeCenter defines the PS variable #1.x and #1.y, which can then
% be used by the user. #1 must be a valid node name
\def\psGetNodeCenter#1{ tx@NodeDict begin /N@#1 load GetCenter end % x y on stack in system coor
  \pst@number\psyunit div /#1.y exch def 	% /#1.y in user coor
  \pst@number\psxunit div /#1.x exch def }	% /#1.x in user coor
%\def\psGetNodeEdgeA#1#2{ tx@NodeDict begin /N@#2 load #2 GetEdgeA end % x y on stack in system coor
%  \pst@number\psyunit div /#1.y exch def 	% /#1.y in user coor
%  \pst@number\psxunit div /#1.x exch def }	% /#1.x in user coor
\def\psGetEdgeA#1#2{
  tx@NodeDict begin \psk@offsetA \psk@offsetB neg 
    \psk@nodesepA \psk@nodesepB 0 0 
    /N@#1 /N@#2 InitNC { NCCoor } if pop pop \tx@UserCoor end}
\def\psGetEdgeB#1#2{
  tx@NodeDict begin \psk@offsetA \psk@offsetB neg 
    \psk@nodesepA \psk@nodesepB 0 0 
    /N@#1 /N@#2 InitNC { NCCoor } if 4 2 roll pop pop \tx@UserCoor end}
%
%%%%%%%%%%%%%% the pst-node-tools part %%%%%%%%%%%%%%%%%%%%%%%%
%
\def\ncbarr{\pst@object{ncbarr}}
\def\ncbarr@i#1#2{%
  \begingroup
  \use@par%
  \psLNode(#1)(#2){0.5}{barr@tempNode}%
  \pst@dimc=\psk@angleA pt
  \pst@dimd=180pt
  % be sure, that angleA is 0 or 180. if not, we set it to 0
  \ifdim\pst@dimc=\z@\else\ifdim\pst@dimc=\pst@dimd\else\psset{angleA=0}\fi\fi
  \ncbar[arrows=-]{#1}{barr@tempNode}
  \ifdim\psk@angleA pt=\z@\relax
    \ncbar[angleA=180,angleB=180]{barr@tempNode}{#2}
  \else\ncbar[angleA=0,angleB=0]{barr@tempNode}{#2}\fi%
  \endgroup%
}
%   #1-------#4----------------#2
% where #1#4= #3 * #1#2
%
\def\psLNode(#1)(#2)#3#4{%
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#2}\pst@tempB%
  \pnode(!
    \pst@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \pst@tempB /YB exch \pst@number\psyunit div def
    /XB exch \pst@number\psxunit div def
    /dx XB XA sub def
    /dy YB YA sub def
    XA dx #3\space mul add YA dy #3\space mul add){#4}}
%
% build the linear combination #2*#1+#4*#3=#5
\def\psLCNode(#1)#2(#3)#4#5{%
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#3}\pst@tempB%
  \pnode(!
    \pst@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \pst@tempB /YB exch \pst@number\psyunit div def
    /XB exch \pst@number\psxunit div def
    XA #2\space mul XB #4\space mul add
    YA #2\space mul YB #4\space mul add){#5}}
%
\def\psLDNode(#1)(#2)#3#4{%  
% #1: node A  #2: node B  #3: dimen measured from A  #4: node name
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#2}\pst@tempB%
  \pssetlength\pst@dimb{#3}%
  \pnode(!%
    \pst@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \pst@tempB /YB exch \pst@number\psyunit div def
    /XB exch \pst@number\psxunit div def
    /dx XB XA sub def
    /dy YB YA sub def
    /angle dy dx Atan def
    /linelength \pst@number\pst@dimb \pst@number\psunit div def
    XA linelength angle cos mul add YA linelength angle sin mul add ){#4}%
}
\def\psRelNode{\pst@object{psRelNode}}
\def\psRelNode@i(#1)(#2)#3#4{{% A - B - factor - node name
  \use@par
%  \pst@killglue
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#2}\pst@tempB%
  \pnode(!
    \pst@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \pst@tempB /YB exch \pst@number\psyunit div def
    /XB exch \pst@number\psxunit div def
    /AlphaStrich \psk@angleA\space def
    /unit \pst@number\psyunit \pst@number\psxunit div def % yunit/xunit
%            
    /dx XB XA sub  def
    /dy YB YA sub \ifPst@trueAngle\space unit mul \fi\space def
    /laenge dy dup mul dx dup mul add sqrt #3 mul def
    /Alpha dy dx atan def 
    /beta Alpha AlphaStrich add def
    laenge beta cos mul XA add
    laenge beta sin mul \ifPst@trueAngle\space unit div \fi\space YA add ){#4}%
}\ignorespaces}
%
\define@cmdkeys[psset]{pstricks-add}[PSTPSPNk@]{% Christophe Jorssen 2007
  blName,bcName,brName,
  clName,ccName,crName,
  tlName,tcName,trName}[]{}%
\psset[pstricks-add]{%
  blName=PSPbl,bcName=PSPbc,brName=PSPbr,
  clName=PSPcl,ccName=PSPcc,crName=PSPcr,
  tlName=PSPtl,tcName=PSPtc,trName=PSPtr}
\def\psDefPSPNodes{\def\pst@par{}\pst@object{psDefPSPNodes}}
\def\psDefPSPNodes@i{%
  \pst@killglue
  \begingroup
  \use@par
  \expandafter\psDefPSPNodes@ii\pic@coor}
%
\def\psDefPSPNodes@ii(#1)(#2)(#3){%
%    \pnode(#1){PSPN@temp}\pnode([nodesep=.75,angle=45]PSPN@temp){\PSTPSPNk@blName}
%    \pnode(#3){PSPN@temp}\pnode([nodesep=.75,angle=-135]PSPN@temp){\PSTPSPNk@trName}
    \pnode(#1){PSPN@temp}\pnode([angle=45]PSPN@temp){\PSTPSPNk@blName}
    \pnode(#3){PSPN@temp}\pnode([angle=-135]PSPN@temp){\PSTPSPNk@trName}
    \pnode(\PSTPSPNk@blName|\PSTPSPNk@trName){\PSTPSPNk@tlName}
    \pnode(\PSTPSPNk@trName|\PSTPSPNk@blName){\PSTPSPNk@brName}
    \ncline[linestyle=none]{\PSTPSPNk@blName}{\PSTPSPNk@tlName}
    \ncput[npos=.5]{\pnode{\PSTPSPNk@clName}}
    \ncline[linestyle=none]{\PSTPSPNk@blName}{\PSTPSPNk@brName}
    \ncput[npos=.5]{\pnode{\PSTPSPNk@bcName}}
    \pnode(\PSTPSPNk@brName|\PSTPSPNk@clName){\PSTPSPNk@crName}
    \pnode(\PSTPSPNk@bcName|\PSTPSPNk@trName){\PSTPSPNk@tcName}
    \pnode(\PSTPSPNk@bcName|\PSTPSPNk@clName){\PSTPSPNk@ccName}
  \endgroup
  \ignorespaces}
%
%
\def\psDefBoxNodes#1#2{\rnode[tl]{#1:tl}{\rnode[Bl]{#1:Bl}{\rnode[tr]{#1:tr}{%
\rnode[bl]{#1:bl}{\rnode[Br]{#1:Br}{\rnode[br]{#1:br}{#2}}}}}}%
\pnode(!\psGetNodeCenter{#1:bl}
          \psGetNodeCenter{#1:tl} 
          #1:bl.x #1:tl.x add 2 div #1:bl.y #1:tl.y add 2 div ){#1:Cl}%
\pnode(!\psGetNodeCenter{#1:tr}
          \psGetNodeCenter{#1:br} 
          #1:tr.x #1:br.x add 2 div #1:tr.y #1:br.y add 2 div ){#1:Cr}%
\pnode(!\psGetNodeCenter{#1:Cl}
          \psGetNodeCenter{#1:Cr} 
          #1:Cl.x #1:Cr.x add 2 div #1:Cl.y #1:Cr.y add 2 div ){#1:C}%
\pnode(!\psGetNodeCenter{#1:Br}
          \psGetNodeCenter{#1:Bl} 
          #1:Br.x #1:Bl.x add 2 div #1:Br.y #1:Bl.y add 2 div ){#1:BC}%
\pnode(!\psGetNodeCenter{#1:tr}
          \psGetNodeCenter{#1:tl} 
          #1:tr.x #1:tl.x add 2 div #1:tr.y #1:tl.y add 2 div ){#1:tC}%
\pnode(!\psGetNodeCenter{#1:br}
          \psGetNodeCenter{#1:bl} 
          #1:br.x #1:bl.x add 2 div #1:br.y #1:bl.y add 2 div ){#1:bC}}%
%
%
%% Author: Michael Sharpe (msharpe at ucsd.edu)
% Macros defined in this file:
% \defaultvalue{<command>}{<value>} assigns <value> to <command> is command is not defined, or is empty.
% \testAlg---used internally to test whether an parametric expression in t is algebraic
% \trim{<command>} trims white space from ends of expansion of <command>
% \hasparen sets \parentrue if its argument contains a (
% \hasequal sets \equaltrue if its argument starts with =
% \equalwhat returns what follows =
% \parsenodexn parses a node expression recursively. Better to use \nodexn.
% \normalvec(<vec>){<nodename>} returns vector normal to <vec> (same length) in <nodename>
% \curvepnode{<t>}{<expression in t>}{<nodename>} Eg, \curvepnode{1}{sin(t) | cos(t)}{P} sets a pnode named P at (cos(1), sin(1))
% \psparnode{<t>}{<expression> in t>}{<nodename>} is called by \curvename if expression is PostScript, not algebraic
% \algparnode{<t>}{<expression> in t>}{<nodename>} is called by \curvename if expression is algebraic, not PostScript
% \nodexn is like \parsenodexn, slightly different syntax. \nodexn{<exn>}{<name>} evaluates <exn> as a node expression and calls the result <name>. 
% \psxline(P){<nodexn1>}{<nodexn2>} draws line from P+<nodexn1> to P+<nodexn2>. The novelty is that the last two arguments can be node expressions.
% \curvepnodes{<tmin>}{<tmax>}{<expression in t>}{<node root name>} Uses current setting of plotpoints (default 50) to define a sequence of pnodes along the curve. Eg, \curvepnodes[plotpoints=100]{0}{1}{t+t^2 | Ex(-t)}{P} sets pnodes P0..P99 at equally spaced t values along the curve, and defines the macro \Pnodecount to 99, the highest index. The expression in t may be either algebraic or PostScript, and is handled automatically detected.
% \fnpnode{<xval>}{<expression in x>}{<nodename>} sets a single pnode on graph. Eg, \fnpnode{.5}{x 2 mul x 1 add mul}{P} declares the pnode P at the point x=0.5 on the graph. (Same as \pnode(!/x 0.5 def x x 2 mul x 1 add mul}){P}.) If your expression in t is algebraic, you must use the keyword algebraic, as in \fnpnode[algebraic]{0.5}{2*x*(x+1)}{P}.
% \fnpnodes{<xmin}{<xmax>}{<expression in x>}{<node root name>} Is exactly the same as \curvenodes, but for the graph of a function. The keyword algebraic must be specified if your expression is algebraic
% \AtoB(A)(B){C} defines node by name C essentially as B-A
% \AplusB(A)(B){C} defines node by name C essentially as A+B
% \midAB(A)(B){C} defines node by name C essentially as (A+B)/2
% \psnline[linewidth=1pt,arrows=->](3,5){P}, for example, expects that there are pnodes named P3..P7 (total of 5), and effectively gives the same result as \psline[linewidth=1pt,arrows=->](P3)(P4)(P5)(P6)(P7). Note that arrow must be specified with a keyword, not as an argument.
% \shownode(P) displays in the console window the coordinates of node P. This will not appear until the final stage of processing the PostScript file. It is a debugging tool.
% \getnodelist{<node root name>}{<next command>} is useful in writing pstricks macros, where there is a list of parenthesized coordinates to be read and turned into a node sequence, following which <next command> is followed.
% \pnodes{P}(1,2)(2;3)... is effectively \getnodelist{P}{}(1,2)(2;3)..., just a quick way to turn a list of coordinates into pnodes P0 P1 ...
% \psLCNodeVar is similar to \psLCNode, and provides a means of forming a linear combination of two nodes, thought of as vectors. Where \psLCNode(A){a}(B){b}{C} effectively makes C=aA+bB, \psLCNodeVar(A)(B)(a,b){C} does the same, but the third argument (a,b) may be specified in PostScript code or any form recognized by \SpecialCoor. Unlike \psLCNode, the name C may be one of A, B.
% \psRelNodeVar is similar to \psRelNode, and provides a means of rotating and changing the length of a line segment AB about A. The effect of \psRelNodeVar(A)(B)(2;30){C} is the same as \psRelNode[angle=30](A)(B){2}{C}, but the third argument (2;30) may be specified in PostScript code, which is not possible with \psRelNode.
% \psRelLineVar stands to \psRelLine as \psRelNodeVar stands to \psRelNode.
% \rhombus{<edge length>}(A)(B){C}{D} computes the two remaining vertices C, D given two opposing vertices A, B of a rhombus with given edge length. It does not draw the rhombus--- that can be handled easily by \pspolygon(A)(C)(B)(D).
% \psrline(P)(Q)... is like \psline, drawing a line starting at (P), with successive increments (Q)... It has the same options as \psline. Eg, \psrline[linecolor=red]{->}(1,1)(1,0)
% \polyIntersection is the most complicated macro in the collection. It has two forms
% \polyIntersection{<Nodename1>}{<Nodename2>}(A)(B)(1,2)(3;30)(6,5)...
%works with the line starting at A heading toward B, and computes the first point that lies on the polyline (1,2)(3;30)(6,5)..., calling it <Nodename1>. It also computes the first point in the opposite direction (from A) lying on that polyline, naming it <Nodename2>. If one or other of these intersections is empty, the nodes are set to remote points on the line. The two nodes are then joined by a line. The effect depends on the location of A and B relative to the polyline, with two cases worth noting.
% (a) if the polyline is closed and if A, B are interior to one of its components, you get a line segment from one edge to the other, containing AB.
% (b) If the polylne is simple and closed, and one of A, B is inside and the other outside, the resulting line segment will contain A but not B. 
% \polyIntersection{<Nodename1>}{<Nodename2>}(A)(B){P}{n} works exactly the same as \polyIntersection{<Nodename1>}{<Nodename2>}(A)(B)(P0)(P1)...(Pn), assuming P0...Pn are previously defined as pnodes.
% \psStepa is like \psStep (pstricks-add) but for a node sequence rather than equally spaced abscissas. \psStepa[options]{<node root>}{<maxindex>} draws a step function with jumps at the successive nodes in the node sequence. Eg, \psStepa{P}{10} has jumps at P0..P10
%
\newcount\pst@args%used in several macros
\newcount\num@pts
\newcount\pst@argcnt% for use in parsing node expressions
\def\PST@root{}
\let\pst@next\relax
%my scratch variables
\def\my@tempA{}
\def\my@tempB{}
\def\my@tempC{}
\def\my@tempD{}
\def\my@next{}
\newif\if@paren%
\newif\if@equal%
\newif\if@colon%
\newif\ifshow
\def\plussign{+}\def\minussign{-}
%
%
\def\defaultvalue#1#2{%#1 is a command, #2 is a value, possibly a command
  \ifdefined#1\ifx#1\@empty\xdef#1{#2}\fi\else\xdef#1{#2}\fi}%
%
\def\testAlg#1|#2\@nil{%
\ifx\relax#2\relax%
   \let\my@next\psparnode\xdef\my@tempD{}%
\else%
   \let\my@next\algparnode\xdef\my@tempD{A}% algebraic
\fi}%
%
%Jonathan Fine's trim
\def\trim #1{\expandafter\trim@\expandafter{#1 }#1}%
\def\trim@ #1{\trim@@ @#1 @ #1 @ @@}%
\def\trim@@ #1@ #2@ #3@@{\trim@@@\empty #2 @}%
\def\unbrace#1{#1}%
\unbrace{\def\trim@@@ #1 } #2@#3{\expandafter\def%
  \expandafter #3\expandafter {#1}}%
%
\def\hasparen#1(#2\@nil{%check if expression contains a (--call with \hasparen#1(\@nil
  \ifx\relax#2\relax \@parenfalse \else \@parentrue\fi}%
%
\def\hasequal#1=#2\@nil{%check if expression contains a =--call with \hasequal#1=\@nil
  \ifx\relax#2\relax \@equalfalse \else \@equaltrue\fi
  \hascolon#2:\@nil}%
%
\def\hascolon#1:#2\@nil{%check if expression contains a :--call with \hascolon#1:\@nil
\ifx\relax#2\relax \@colonfalse \else \@colontrue\fi}%
%
\def\equalwhat#1=#2:#3\@nil{{#2}{#3}}%
%
\def\parsenodexn#1(#2)#3\@nil{%
  \def\coeffA{#1}\edef\nodeA{#2}%
  \trim\coeffA%
  \ifx\nodeA\@empty\else%
    \pnode(#2){@@TMP}%
    \ifx\coeffA\@empty\def\coeffA{1}\else%
      \ifx\coeffA\plussign\def\coeffA{1}\else\ifx\coeffA\minussign\def\coeffA{-1}\fi\fi\fi% 
  \edef\cmd{\noexpand\psLCNode(@TMP\the\pst@argcnt){1}(@@TMP){\coeffA}{@TMP}}%
  \cmd%
  \advance\pst@argcnt by \@ne%
  \pnode(@TMP){@TMP\the\pst@argcnt}%
  \parsenodexn#3\@nil%
  \fi}%
%
\def\normalvec(#1)#2{%
%pnode | new pnode normal to old, same  length
  \psRelNodeVar(0,0)(#1)(0,1){#2}}%
%
\def\curvepnode#1#2#3{%
% #1=t value, #2=x(t) y(t) in either form,#3=node name,
%must first detect which form of x(t) y(t), looking for |
  \edef\my@tempA{#2}% x(t) y(t) expanded
  \expandafter\testAlg\my@tempA|\@nil\my@next {#1}{#2}{#3}}
%
\def\psparnode#1#2#3{%
% #1=t value, #2=x(t) y(t) in PS form,#3=node name,
  \pnode(!/t #1 def #2){#3}%
  \pnode(!/t #1 .001 sub def #2 
          /t #1 .001 add def 
           #2 3 -1 roll sub 3 1 roll sub neg 
           2 copy Pyth dup 3 1 roll div 3 1 roll div ){#3tang}}%unit tangent vector at t
%
\def\algparnode#1#2#3{%
% #1=t value, #2=x(t) | y(t) in alg form,#3=node name,
%\pstVerb{tx@Dict begin /t #1 def /Func (#2) AlgParser cvx def end}
%\pnode(!Func){#3}}%
  \pstVerb{tx@Dict begin /Func (#2) AlgParser cvx def end }
  \pnode(!/t #1 def Func){#3}
  \pnode(!/t #1 .001 sub def Func 
          /t #1 .001 add def 
          Func 3 -1 roll sub 3 1 roll sub neg 
          2 copy Pyth dup 3 1 roll div 3 1 roll div ){#3tang}%unit tangent vector at t
}%
%
\def\nodex#1{%
%#1=node expression --set nodename to @TMP
\expandafter\hasparen#1(\@nil%
\if@paren%it's an expression
  \pnode(0,0){@TMP0}%
  \pst@argcnt=0%
  \expandafter\parsenodexn#1()\@nil%
\else%
  \def\my@tempC{#1}%
  \ifx\my@tempC\@empty\pnode(0,0){@TMP}\else\pnode(#1){@TMP}\fi%
\fi}%\if@paren
%
\def\nodexn#1#2{%
%#1=node expression | #2=node name
\expandafter\hasparen#1(\@nil%%%      hv 20130917 use \expandafter
\if@paren%it's an expression
  \pnode(0,0){@TMP0}%
  \pst@argcnt=0%
  \parsenodexn#1()\@nil%
  \pnode(@TMP){#2}%
\else%
  \def\my@tempC{#1}%
  \ifx\my@tempC\@empty\pnode(0,0){#2}\else\pnode(#1){#2}\fi%
\fi}%\if@paren
%
\def\psxline{\pst@object{psxline}}%
\def\psxline@i{\@ifnextchar({\psxline@iii}{\psxline@ii}}%
\def\psxline@ii#1{%
\addto@par{arrows=#1}%
\psxline@iii}%
\def\psxline@iii(#1)#2#3{{%#1=basepoint, #2,#3 node expressions
\pst@killglue%
\use@par%
\nodexn{#2}{@TMP@a}%
\AplusB(#1)(@TMP@a){@TMP@A}%
\nodexn{#3}{@TMP@a}%
\AplusB(#1)(@TMP@a){@TMP@B}%
\psline(@TMP@A)(@TMP@B)%
}%
\ignorespaces}%
%
\def\curvepnodes{\pst@object{curvepnodes}}
\def\curvepnodes@i#1#2#3#4{{%optional [plotpoints=xx]
%  #1=tmin,#2=tmax,#3=function (of t),#4=node root name,
  \pst@killglue
  \use@par
  \edef\my@tempA{#3}% x(t) y(t) expanded
  \expandafter\testAlg\my@tempA|\@nil %
  \pstVerb{% 
	tx@Dict begin % so we can use definitions from tx@Dict
	/t0 #1 def
	/t1 #2 def  
	 t1 t0 sub end \psk@plotpoints div /dt exch def }%
  \pst@cntc=\psk@plotpoints\relax%\psk@plotpoints=plotpoints-1
  \advance\pst@cntc by \@ne\relax %=plotpoints
  \ifx\my@tempD\@empty\pstVerb{tx@Dict begin /Func (#3) cvx def end }%add tx@Dict
  \else\pstVerb{tx@Dict begin /Func (#3 ) AlgParser cvx def end }%
  \fi%
    \multido{\i=0+1}{\pst@cntc}{%
      \pnode(! /t #1 dt \i\space mul add def Func ){#4\i}}% remove t before Func
    \expandafter\xdef \csname #4nodecount\endcsname {\psk@plotpoints}%
    \ifnum\Pst@Debug>0 \typeout{Created nodes #40 .. #4\psk@plotpoints}\fi%
}\ignorespaces}%
%
\def\fnpnode{\pst@object{fnpnode}}
\def\fnpnode@i#1#2#3{{%optional [algebraic]
%#1=x value | #2=fn of x | #3=node name
  \pst@killglue
  \use@par
  \ifPst@algebraic\pnode(*#1 {#2}){#3}\else\pnode(! /x #1 def x #2){#3}\fi
}\ignorespaces}%
%
\def\fnpnodes{\pst@object{fnpnodes}}
\def\fnpnodes@i#1#2#3#4{{%optional [algebraic]
%#1=xmin | #2=xmax | #3= fn of x | #4=node name
\pst@killglue
\use@par
\pst@dima=#1pt \pst@dimb=#2pt \advance\pst@dimb -\pst@dima%
\pst@cnta=\psk@plotpoints \relax %=plotpoints-1
\def\PST@root{#4}
\divide\pst@dimb by \pst@cnta%plotpoint-1 intervals
\pst@cntc=\pst@cnta %
\advance\pst@cntc by 1 \relax %=plotpoints
\ifPst@algebraic 
  \multido{\i=0+1}{\pst@cntc}{\pnode(*{\pst@number\pst@dima} {#3}){#4\i}%  hv 20130713
  \advance\pst@dima \pst@dimb}%
\else
    \multido{\i=0+1}{\pst@cntc}{\pnode(!/x \pst@number\pst@dima\space def x #3){#4\i}%
  \advance\pst@dima \pst@dimb}%
\fi%
  \expandafter\xdef \csname \PST@root nodecount\endcsname {\the\pst@cnta}%
  \ifnum\Pst@Debug>0 \typeout{Created nodes #40 .. #4\the\pst@cnta}\fi%
}\ignorespaces}%
%
\def\AtoB(#1)(#2)#3{\psLCNodeVar(#1)(#2)(-1,1){#3}}
\def\AplusB(#1)(#2)#3{\psLCNodeVar(#1)(#2)(1,1){#3}}
\def\midAB(#1)(#2)#3{\psLCNodeVar(#1)(#2)(.5,.5){#3}}
%
\def\psnline{\pst@object{psnline}}%line of nodes
\def\psnline@i{\pst@getarrows{\psnline@ii}}
\def\psnline@ii(#1,#2)#3{{%
\pst@killglue%
\use@par%
\pst@cnta=#2 \relax\advance\pst@cnta by 1
\edef\@tmp{}%
\multido{\i=#1+1}{\pst@cnta}{\xdef\@tmp{\@tmp(#3\i)}}%
\expandafter\psline\@tmp}%
\ignorespaces}%
%
\def\psncurve{\pst@object{psncurve}}%line of nodes
\def\psncurve@i{\pst@getarrows{\psncurve@ii}}
\def\psncurve@ii(#1,#2)#3{{%
\pst@killglue%
\use@par%
\pst@cnta=#2 \relax\advance\pst@cnta by 1
\edef\@tmp{}%
\multido{\i=#1+1}{\pst@cnta}{\xdef\@tmp{\@tmp(#3\i)}}%
\expandafter\pscurve\@tmp}%
\ignorespaces}%
%
\def\psnccurve{\pst@object{psnccurve}}%line of nodes
\def\psnccurve@i{\pst@getarrows{\psnccurve@ii}}
\def\psnccurve@ii(#1,#2)#3{{%
\pst@killglue%
\use@par%
\pst@cnta=#2 \relax\advance\pst@cnta by 1
\xdef\@tmp{}%
\multido{\i=#1+1}{\pst@cnta}{\xdef\@tmp{\@tmp(#3\i)}}%
\expandafter\psccurve\@tmp}%
\ignorespaces}%
%
\def\shownode(#1){%display node user coords in console
  \pst@killglue%
  \pstVerb{% 
    gsave tx@Dict begin %
    tx@NodeDict /N@#1 known { % known node
      /tmpar [(Node #1: ) <28> () (, ) () <29>] def %
      /str 12 string def 
      STV CP T \psGetNodeCenter{#1}\space 
      tmpar 2 #1.x str cvs put 
      /str 12 string def 
      tmpar 4 #1.y str cvs put 
      tmpar concatstringarray = }%
    {% not known
      (Node #1: (NOT KNOWN)) = %
    } ifelse %
    end grestore }%
  \ignorespaces}%
%
% Use to construct a sequence of nodes
% Eg, \pnodes{P}(0,1)(2;5)(3,4) defines nodes P0, P1, P2 with respective locations
% and a macro \Pnodecount containing the highest index created
\def\pnodes@ii#1{\getnodelist{#1}{}}
%
\def\getnodelist#1#2{%
\pst@args=0 \relax%
\def\PST@root{#1}%
\def\pst@next{#2}% command to perform after reading list
\getnext@Node}%
%
\def\getnext@Node{\@ifnextchar({\getnext@Node@i}%
  {\advance\pst@args by \m@ne \expandafter\xdef \csname \PST@root nodecount\endcsname {\the\pst@args}
  \ifnum\Pst@Debug>0 \typeout{Created nodes \PST@root0 .. \PST@root\the\pst@args}\fi% 
  \pst@next}%
}%
%
\def\getnext@Node@i(#1){%
\pnode(#1){\PST@root\the\pst@args}%
\advance\pst@args by \@ne\relax%
\getnext@Node}%
%
\def\psLCNodeVar(#1)(#2)(#3)#4{%
\pst@getcoor{#1}\my@tempA%
\pst@getcoor{#2}\my@tempB%
\pnode(#3){tmpLCn@de}%
\pnode(!%
  \my@tempA /YA exch \pst@number\psyunit div def
  /XA exch \pst@number\psxunit div def
  \my@tempB /YB exch \pst@number\psyunit div def
  /XB exch \pst@number\psxunit div def %stack now empty
  \psGetNodeCenter{tmpLCn@de}\space
  XA tmpLCn@de.x mul XB tmpLCn@de.y mul add
  YA tmpLCn@de.x mul YB tmpLCn@de.y mul add){tmpLCn@deA}%
\pnode(tmpLCn@deA){#4}%
}%
%
\def\psRelNodeVar{\pst@object{psRelNodeVar}}
\def\psRelNodeVar@i(#1)(#2)(#3)#4{{% A - B - factor;angle - node name
  \use@par
  \pst@getcoor{#1}\my@tempA%
  \pst@getcoor{#2}\my@tempB%
   \pnode(#3){tmpn@de}%
\pnode(!
  /unit \pst@number\psyunit \pst@number\psxunit div def % yunit/xunit
    \my@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \my@tempB /YB exch \pst@number\psyunit div YA sub 
    \ifPst@trueAngle\space unit mul \fi\space def
    /XB exch \pst@number\psxunit div XA sub def
    %complex multiply (XB,YB) and (P.x,P.y), then add (XA,YA)
    \psGetNodeCenter{tmpn@de}
    XB tmpn@de.x mul YB tmpn@de.y mul sub
    YB tmpn@de.x mul XB tmpn@de.y mul add
    \ifPst@trueAngle\space unit div \fi\space 
   YA add exch XA add exch %x, y coords on stack
    ){#4}%
}}
%
\def\psRelLineVar{\pst@object{psRelLineVar}}
\def\psRelLineVar@i{\@ifnextchar({\psRelLineVar@iii}{\psRelLineVar@ii}}
\def\psRelLineVar@ii#1{%
  \addto@par{arrows=#1}%
  \psRelLineVar@iii}
\def\psRelLineVar@iii(#1)(#2)(#3)#4{{%
  \pst@killglue
  \use@par
  \psRelNodeVar(#1)(#2)(#3){#4}%
  \psline(#1)(#4)%
}\ignorespaces}
%
\def\rhombus#1(#2)(#3)#4#5{% \rhombus{m}(B)(D){A}{C} 
\AtoB(#2)(#3){node@P}% P=BD
% compute angle between BD and BC, in Postscript
\pnode(! %compute angle and scale in PS
/tmp \psGetNodeCenter{node@P} node@P.x node@P.y 
Pyth 2 div def %tmp=half-length of BD
/ang tmp #1\space div Acos def %ang=angle from BD to BC & BA
#1\space tmp 2 mul div %scale factor s=m/BD
dup ang cos mul exch ang sin mul ){node@A1}% s cos(ang), s sin(ang)
\pnode(! \psGetNodeCenter{node@A1} node@A1.x node@A1.y neg ){node@A2}%reflect in x axis
\psRelNodeVar(#2)(#3)(node@A1){#4}%
\psRelNodeVar(#2)(#3)(node@A2){#5}%
}%
%
\def\psrline{\pst@object{psrline}}% relative lines
\def\psrline@i{\@ifnextchar({\psrline@iii}{\psrline@ii}}%
\def\psrline@ii#1{%
\addto@par{arrows=#1}%
\psrline@iii}%
\def\psrline@iii{%
\getnodelist{@tmpnode}{\psrline@iv}%
}%
\def\psrline@iv{%
   \ifnum\pst@args<0\else%do nothing
      \pnode(@tmpnode0){@tmpnodeB0}%
      \multido{\iA=1+1,\iB=0+1}{\pst@args}{%
      \AplusB(@tmpnodeB\iB)(@tmpnode\iA){@tmpnodeB\iA}}%
      \psrline@v%
   \fi%
}%
\def\psrline@v{{%finish up
  \pst@killglue%
  \use@par%
  \xdef\tmp{(@tmpnodeB0)}%
  \multido{\i=1+1}{\pst@args}%
{\xdef\tmp{\tmp(@tmpnodeB\i)}}%
\expandafter\psline\tmp%
}\ignorespaces}%
%
\def\polyIntersections#1#2(#3)(#4){%
%nodename1 | nodename2 | A | B | % intersections with line from A, B 
\def\nodenameA{#1}\def\nodenameB{#2}%
\pnode(#3){P@A}\pnode(#4){P@B}%
\@ifnextchar({\polyIntersections@next}{\polyIntersections@ii}%
}%
\def\polyIntersections@ii#1#2{%
\def\root@node{#1}\num@pts=#2 \relax%
\polyIntersections@iii}% 
%
\def\polyIntersections@next{%read as many points as exist
\def\root@node{P@}\getnodelist{P@}{\num@pts=\pst@args \relax\polyIntersections@iii}%
}%
\def\polyIntersections@iii{%nodes are now XXX0....XXXn, n=num@pts
\pst@cnta=\num@pts \relax\advance\pst@cnta by 1 \relax%
\pstVerb{%
 /xarray \the\pst@cnta\space array def
 /yarray \the\pst@cnta\space array def  tx@Dict begin }%
\multido{\i=0+1}{\the\pst@cnta}{\pstVerb{ \psGetNodeCenter{\root@node\i} xarray \i\space \root@node\i.x put yarray \i\space \root@node\i.y put }}%
\pstVerb{ /tposmin 100 def /tnegmax -100 def %/argposmin 0 def /argposmax 0 def 
\psGetNodeCenter{P@B} \psGetNodeCenter{P@A} 
/dx P@B.x P@A.x sub def 
/dy P@B.y P@A.y sub def 
/lenAB dx dy Pyth def
/oldx xarray 0 get def /oldy yarray 0 get def 
1 1 \the\num@pts\space {/k exch def /newx xarray k get def /newy yarray k get def 
/ddx newx oldx sub def /ddy newy oldy sub def 
/det ddy dx mul ddx dy mul sub def
det abs lenAB ddx ddy Pyth mul .001 mul gt 
{/ac oldx P@A.x sub def /bd oldy P@A.y sub def 
 /tt  ac ddy mul bd ddx mul sub det div def %solve for t value at intersection
 /ss ac  dy mul bd dx mul sub det div def % solve for s value at intersection
ss 0 ge 
   {ss 1 le 
        {tt 0 lt {tt tnegmax gt {/tnegmax tt def} if } {tt tposmin lt {/tposmin tt def} if } ifelse }
    if } % ss 1 le
if }%ss 0 ge
 if %det>
 /oldx newx def /oldy newy def} for end }%
\pnode(! \psGetNodeCenter{P@A} \psGetNodeCenter{P@B} P@B.x P@A.x sub  tposmin mul P@A.x add  P@B.y P@A.y sub tposmin  mul P@A.y add ){\nodenameA}%
\pnode(! \psGetNodeCenter{P@A} \psGetNodeCenter{P@B} P@B.x P@A.x sub tnegmax mul P@A.x add P@B.y P@A.y sub tnegmax mul P@A.y add){\nodenameB}%
}%
%
\def\actualscale#1 #2 scale{% extract x-scale from, eg,  {2. 2. scale}
#1}
%
\def\psGetCenter#1{ tx@NodeDict begin /N@#1 load GetCenter end }% x y on stack in system coor
%
\def\ArrowNotch{\pst@object{ArrowNotch}}
\def\ArrowNotch@i#1#2#3#4{{%
%noderootname | index | arrowdirection | notchnodename  % 
\pst@killglue%
\use@par%
\def\inc{-1}%
\ifx#3<\def\inc{1}\fi% -1 means notch to left of arrowhead
%get length of pointed arrow under these conditions (types ->, -D> and their reverses)
\pstVerb{ 
    1 \psk@arrowinset\space sub \psk@arrowlength\space \psk@arrowsize\space  
    \pst@number\pslinewidth \space mul add  mul mul 
    \expandafter\actualscale\psk@arrowscale \space  mul 
    /hh exch def /hh1 hh .05 sub def }% PS variable hh contains dist from tip to notch of arrow, in pts
\def\root@node{#1}\num@pts=\csname\root@node nodecount\endcsname %
\pst@cntb=\num@pts \advance\pst@cntb by \@ne%actual node count
\pst@cnta=\num@pts \advance\pst@cnta by \thr@@%size of PS array
\pst@cntc=#2 \relax% index of center of circle
\ifnum\pst@cntc>\num@pts \pnode(0,0){#4}\else
%compute a (screen based) unit vector in directions P1P0 and Pn-1Pn
\pstVerb{%
/PythSq { dup mul exch dup mul add } def
/PtSub {					%  xA yA xB yB
  3 -1 roll 		% xA xB yB yA
  sub neg		% xA xB yA-yB
  3 1 roll 		% yB-yA xA xB
  sub			% yB-yA xA-xB
  exch                     % xB-xA yA-yB
} def
  /xarray \the\pst@cnta\space array def
  /yarray \the\pst@cnta\space array def  
  tx@Dict begin }% end pstVerb
\multido{\i=0+1,\ib=1+1}{\the\pst@cntb}{\pnode(! \psGetCenter{\root@node\i}\space  % center on stack in system coords, not user coords
yarray \ib\space 3 -1 roll put xarray \ib\space 3 -1 roll put 0 0 ){@tmp}}% end multido
%\pstVerb{ \psGetCenter{\root@node6} == == }
\pnode(! xarray 1 get dup yarray 1 get dup 3 1 roll % x1 y1 x1 y1
xarray 2 get yarray 2 get PtSub  % x1 y1 x1-x2 y1-y2
2 copy Pyth hh div 2 div dup % x1 y1 x1-x2 y1-y2 d d ,d->d/2*hh
3 1 roll % x1 y1 x1-x2 d y1-y2 d
div 3 1 roll div %x1 y1  (y1-y2)/d (x1-x2)/d
3 1 roll %x1  (x1-x2)/d y1  (y1-y2)/d
add 3 1 roll add %  y1-(y2-y1)/d x1-(x2-x1)/d
 xarray 0 3 -1 roll put yarray 0 3 -1 roll put %stack empty
 xarray length 2 sub /topnum exch def 
 xarray topnum get dup yarray topnum get dup 3 1 roll %xn yn xn yn
topnum 1 sub /topnum exch def xarray topnum get yarray topnum get % xn yn xn yn x(n-1) y(n-1)
3 -1 roll sub  neg 3 1 roll sub exch % xn yn (xn-x(n-1)) (yn-y(n-1))
2 copy Pyth hh div 2 div dup % xn yn (xn-x(n-1)) (yn-y(n-1)) d d (d->d/(2*h))
3 1 roll div 3 1 roll div %xn yn (xn-x(n-1))/d (yn-y(n-1))/d
3 -1 roll add 3 1 roll % y(n+1) x(n+1)
topnum 2 add /topnum exch def xarray topnum 3 -1 roll put yarray topnum 3 -1 roll put % empty
% next step--find first index outside circle of radius hh 
 /oldcindex \the\pst@cntc\space 1 add def %position in array
 xarray oldcindex get /xc exch def yarray oldcindex get /yc exch def
 %hh .05 sub /hh exch def % that's close enough for a crossing
/inc \inc\space def %+1 for left facing arrow, else -1 
/cindex oldcindex def 
{cindex inc add /cindex exch def xarray cindex get xc sub yarray cindex get yc sub Pyth dup hh1 gt 
{ exit } if } loop % exit from loop with cindex the first index of an external point--dist on stack
 hh1 .1 add lt { xarray cindex get yarray cindex get } %else within segment
{ xarray cindex inc sub get dup yarray cindex inc sub get dup 4 -1 roll exch 
xarray cindex get yarray cindex get PtSub /dy1 exch def /dx1 exch def dx1 dy1 PythSq /Aterm exch def 
% dx1=x(n-1)-x(n), dy1=y(n-1)-y(n) [if inc=1]: dx1=x(n+1)-x(n), dy1=y(n+1)-y(n) [if inc=-1]
% x(n-inc) y(n-inc),  Aterm=dx1^2+dy1^2
 2 copy xc yc PtSub % x(n-inc) y(n-inc) (x(n-inc)-xc) (y(n-inc)-yc)
 2 copy 2 copy 3 -1 roll mul 3 1 roll mul add hh dup mul sub % x(n-inc) y(n-inc) (y(n-inc)-yc) (x(n-inc)-xc) (x(n-inc)-xc)^2+(y(n-inc)-yc)^2-hh^2
 Aterm div /Cterm exch def  % x(n-inc) y(n-inc)  (y(n-inc)-yc) (x(n-inc)-xc) , Cterm=((x(n-inc)-xc)^2+(y(n-inc)-yc)^2-hh^2)/(Aterm) (<0)
 dx1 dy1 %  x(n-inc) y(n-inc) (y(n-inc)-yc)  (x(n-inc)-xc)  dx1 dy1
 4 1 roll mul 3 1 roll mul add Aterm div /Bterm exch def %   x(n-inc) y(n-inc) , Bterm=( (x(n-inc)-xc)*dx1+(y(n-inc)-yc)*dy1)/Aterm
 Bterm abs neg dup dup mul Cterm sub sqrt add dup /tval exch def
% x(n-inc) y(n-inc) tvalue
 dup dx1 dy1 4 1 roll mul 3 1 roll mul  % x(n-inc) y(n-inc) t*dx1 t*dy1
 PtSub } ifelse % x y screen coords of arrow notch now on stack---convert to user x y
 \pst@number\psyunit div exch \pst@number\psxunit div exch  %use coords now on stack
){#4}\fi%
\pstVerb { end } %tx@Dict
}\ignorespaces}%
%
\def\saveDataAsNodes#1#2{%  Filename NodePrefix
  \psLoopIndex=0\relax
  \typeout{Open file #1}%
  \openin7=#1
  \loop
    \read7 to \@Data
    \ifeof7\else
      \ifx\@Data\@empty\else\pnode(!\@Data){#2\the\psLoopIndex}%
        \typeout{#2\the\psLoopIndex -> \@Data}%
	\advance\psLoopIndex by 1
      \fi
  \repeat
  \closein7
}
%
\catcode`\@=\TheAtCode\relax
\endinput
%%
%% END pst-node.tex

